Policy Optimization in Control: Geometry and Algorithmic Implications

This survey explores the geometric perspective on policy optimization within the realm of feedback control systems, emphasizing the intrinsic relationship between control design and optimization. By adopting a geometric viewpoint, we aim to provide a nuanced understanding of how various ``complete parameterization'' -- referring to the policy parameters together with its Riemannian geometry -- of control design problems, influence stability and performance of local search algorithms. The paper is structured to address key themes such as policy parameterization, the topology and geometry of stabilizing policies, and their implications for various (non-convex) dynamic performance measures. We focus on a few iconic control design problems, including the Linear Quadratic Regulator (LQR), Linear Quadratic Gaussian (LQG) control, and $\mathcal{H}_\infty$ control. In particular, we first discuss the topology and Riemannian geometry of stabilizing policies, distinguishing between their static and dynamic realizations. Expanding on this geometric perspective, we then explore structural properties of the aforementioned performance measures and their interplay with the geometry of stabilizing policies in presence of policy constraints; along the way, we address issues such as spurious stationary points, symmetries of dynamic feedback policies, and (non-)smoothness of the corresponding performance measures. We conclude the survey with algorithmic implications of policy optimization in feedback design.

==> brainstorming-notes.tex <==

\newpage

\section*{Notes on points that need to be reflected in the survey ... }


\section*{group inputs}
Undoubtedly, optimal control and learning of dynamical systems lies at the core of numerous advancements in sequential decision making within systems and control engineering. Over time, optimal control has undergone extensive study in diverse setups and applications, yielding fundamental results through variational techniques [\shahriar{Pontryagin Principle}] and dynamic programming [\shahriar{HJB}] for characterizing ``optimal policies''--mapping the observations of the internal dynamics to control actions that are optimal with respect to a system-level performance measure. In contrast to these methods that are built upon the knowledge of the underlying dynamics, reinforcement learning and adaptive dynamic programming \shahriar{[cite, Lewis and Vrabi]} aim to obtain these optimal policies directly by leveraging the data trajectories of the underlying system dynamics--rather than an ``uncertainty equivalence'' approach\footnote{\shahriar{Uncertainly equivalence refer to...}}. Notably, among these methods, \ac{PO} has emerged as exceptionally effective, finding application across various domains, from \shahriar{(provide examples) to (continue listing examples)}, where policies are often parameterized within a tractable class and subsequently optimized based on system-level performance measures.


the rest of paragraphs:
\begin{itemize}
    \item A paragraph on properties/advantages of \ac{PO} including its applicability in general to various linear/non-linear frameworks, ... a bridging between control and optimization techniques that can be used. this connects to optimization techniques. However, we can point out the complications including, non-convexity of the cost and the domain, parameterization-dependent performance due to the implicit Euclidean geometry often accompanying each parameterization, and conditioning issues due to these parameterization....

    \item This paragraph aims to promote geometric methods from Riemannian optimization by introducing an appropriate metric. We can also formalize what we mean by ``complete parameterization'' and possibly restrict the treatment of this paper to the Linear-Quadratic case. \yang{Probably, we can deal with linear dynamics + quadratic performance, in the presence of either stochastic noises (which is LQR/LQG) or adversarial noises (which corresponds to $\mathcal{H}_\infty$ control). The latter case also has direct implications in robustness and safety for dynamical systems.} \shahriar{It may also makes sense to talk about \citep{nesterov_riemannian_2002}}.

    \item We might need a short paragraph to clarify the differential-geometric techniques in control following the works of Brockett, Wonham and others, and explain that the further interplay between geometric PO and these geometric control approaches will be differed to our future work. \yang{This paragraph will be good and important. It will bring back some earlier control literature and put this survey into a larger context.} \shahriar{That's exactly what I had in mind...indeed this will inspire us to start developing the connection :D }


    \item Moving on with complete parameterization, we point out that different parameterization indeed have different implications on the feasible domain and optimization landscape. In this work we present a few different parameterization with their accompanying Riemannian geometry including static state feedback, static output feedback, and dynamic output feedback. We can further introduce some of the main notation and summarize the topological properties of static feedback \citep{bu_topological_2021} and dynamic feedback \citep{tang_analysis_2021} before moving on to the next point:\\

\end{itemize}



\section*{MM attempt at the intro/outline ... will fold in all the points/paragraphs contributed by the group ...}

Rewrite: Optimization and control theory: closely connected, in fact, since
Kalman's work the relationship has become official through the notion of
optimal control, viewing control design as an optimization problem. 
In hindsight this is not surprising as similar to other engineering disciplines,
control design is most naturally viewed as optimizing the selecting of design parameters in order to achive the design objectives. On the other hand, control theoretic techniques have influence both the design and analysis of optimization algorithms, where the algorithm is viewed as dynamical system that traverses the design landscape to take an initial condition to the optimum- references- old a new.
The relationship however has not been an equal partnership- optimization has had much more influence on control over the past few decades than vice versa- and with all the advances in optimization and ML, this influence will only strengthen.

Segue to feedback design and then policy ... and then new perspectives. 

Embracing the optimization perspective on feedback design: systematic approach in optimization (more specifically in convex optimization) starts with the notion of the constraint set: convex, compact, polyhedral, etc. what features the constraint set has ... then off to functions, convexity, lower, upper approximations, role of Lipschitz continuity, differentiability, convexity, etc. How the function interacts with the set (linear functions are optimized at the boundary- implications for algorithms, e.g, simplex), interior point algorithms/self-concordant barriers, 
lower bound complexity.

The situation in control has been a bit less systematic- and the recent interest in data-driven control, etc. has only made this more pronounced ... in fact, one of the issue that this new perspective has highlighted is the need to re-examine control synthesis in new light and in the process, understand the underlying geometry- full circle back to how optimization theory is often presented ... sets, functions, properties, how they interact, and how such an interaction can lead to design algorithms. so that is the route that we will take.

What do we mean by geometry of policy optimization- how does this relate to various ``geometric'' adverbs that has been added to various approaches to control design. Geometric control, geometric linear system, geometric-algebraic .... 
what is different ... highlight of ``other'' geometric insights- what was the motivation for these works? Geometric linear system aims to make linear control theory coordinate free- analogous to vector space machinery and linear algebra- as such, subspace geometry of various system-theoretic construct become the focus of the work- geometric nonlinear control on the other hand aims to extend linear control to nonlinear settings thru differential geometric methods- e.g., what is the the right way to think about the controllability rank condition for nonlinear systems, etc. our work is motivated by connections to ML/AI/optimization and developing algorithms directly on the policy, and also extending control theory beyond the confinement of LMIs :-) what synthesis procedures- are fundamentally- can be reduced to LMIs?

we pursue this program: stabilizing feedback gains, state/output, the role played by minimality, boundary of the set of state feedback gains, dynamic feedback, ..., natural metrics on the set of stabilizing feedback gains, non-convexity, 
then the objective, PL, non-smooth cases, stationary points, 

The outline of the survey is as follows: optimal control with emphasis on policy- why policy is both interesting, relevant, and why it is tricky- RL perspective- the first type of questions are topological: connectedness, boundary, etc. then move on to the main part that highlights the differential geometric perspective, cost structure, smoothness question, output feedback vs. state feedback, quotient manifolds, ... also thinking about the road ahead, conditioning, towards a more systematic approach to model-based/model free and anything in between!


\newpage

roughly: why geometry matters- a deeper connection between optimization and control--
fundamental limits. each parameterization has its unique geometry,
computational implications, conditioning, and pitfalls. parameterization
leads to new questions and approaches that seem inaccessible in another parameterization.
control theory is old, yet also new. things are not as people like you to believe :-)

may be in the introduction we can talk about topological issues- Jingjing work,
etc. and other related topics- 

\shahriar{What do we mean by geometry?}\\

\textbf{Spencer}: After reading some of the classical references, there seems to be two competing (and overlapping" definitions for "geometry"
\textbf{(1) Coordinate-invariant properties}:
\begin{itemize}
    \item \citep{wonham_w_murray_linear_1985}, \citep{beckmann_invariants_1976}, \citep{byrnes_fine_1980}, \citep{tannenbaum_invariance_1981}, \citep{brockett_early_2014}
    \item defining the system matrices $A\colon\mathcal{X} \to \mathcal{X}$, $B\colon\mathcal{U} \to \mathcal{X}$, $C\colon\mathcal{X} \to \mathcal{Y}$ as abstract linear maps, no basis
    \begin{itemize}
        \item (Wonham) Controllability, observability, stabilization are independent the basis of the spaces $\mathcal{X},\mathcal{U},\mathcal{Y}$, depend solely on subspaces induced from $A,B,C$
    \end{itemize}
    \item in the context of input-output systems: the PO algorithm or cost function does not concern the coordinates of the internal state (i.e. LQG, $H_\infty$ are coordinate-invariant)
    \item instead of state-space realizations, we have orbits of state-space realizations (Kalman, Hazelwinkel, Bynres used Alg-Geo language and referred to these as Moduli spaces)
\end{itemize}

\textbf{(2) Properties of a set or function that is invariant under diffeomorphism}:
\begin{itemize}
    \item \citep{brockett_geometric_1976}
    \item smoothness, number of connected components
    \item geodesic convexity, rate of convergence via RGD
    \item stationary points and their index (i.e. eigenvalue signs)
\end{itemize}










\vspace{1cm}
\textbf{Just a tentative outline for the rest of the paper:} (please feel free to introduce any change here)
\begin{itemize}
    \item The main story around the topology and geometry of policy optimization in control- including a historical points of view. {\color{red} What are the relevant papers in classical control? It would be good to collect a few historical papers; so we can begin to digest them and put those historical perspectives into the current view.
    
    The following bullet points are more recent developments. As indicated above, the geometry and topology are highly dependent on the controller parameterization: static state feedback policies, static output feedback policies, dynamic output feedback policies in the state-space form or the transfer function domain. Different parameterizations have different implications on the feasible region as well as on the landscape of objective functions. 
    }

    
    \item on topology of the set of stabilizing controllers \citep{bu_topological_2021}
    \item on geometry of the static set of stabilizing controllers \citep{talebi_policy_2023}
    \item on geometry of dynamic controllers \citep{tang_analysis_2021}; Yang's recent works
    \item orbit geometry and quotient manifolds//Spencer and Mehran
    
    classical relevant papers:
    \begin{itemize}
        \item \citep{brockett_geometric_1976, tannenbaum_invariance_1981, wonham_w_murray_linear_1985, byrnes_fine_1980}
        \item \citep{tannenbaum_invariance_1981} This textbook studies the algebraic-geometric properties of $\mathcal{L}_{n,m,p}$, the quotient space of state-space representations of $m$-input, $p$-output linear systems modulo coordinate-transformation. This textbook goes heavy into the algebraic-geometry of the topic, not focusing too much on the manifold-ness of $\mathcal{L}_{n,m,p}$
        \item \citep{wonham_w_murray_linear_1985} This textbook defines linear system theory and linear control theory in a geometric (i.e. coordinate-free, basis-free) way. Observability and controllability can be entirely defined in terms of the subspaces induced by $A,B,C$, such as their kernels and images. When a feedback gain $K \in \mathbb{R}^{m \times n}$ is stabilizing, this can be defined just by those subspaces.
        \item \citep{byrnes_fine_1980} this paper focuses on the differential geometric (i.e. manifolds) properties of $\mathcal{L}_{n,m,p}$, unlike \citep{tannenbaum_invariance_1981} who only focuses on the algebraic-geometry. I find this approach far more clean and simple and the alg-geo approach. The remarkable theorem from this paper is that there is no global parameterization of $\mathcal{L}_{n,m,p}$ when $\min(m,p) \geq 2$. 
        \item \citep{brockett_geometric_1976} this paper studies the topological and geometric (i.e. invariant under diffeomorphism) properties of the space of SISO transfer functions with $n$ poles. Brockett shows that there are $n+1$ connected components, determined by the Cauchy index of the transfer function. Brockett also raises other interesting questions. 
    \end{itemize}

    \item interactions between the  constraints

    \item geometry of the performance indices amounting to non-smoothness, to what extend? depending on the space
    
    \item future directions and outlook
\end{itemize}

Let $P$ be our plant, represented as an LTI system. Let $\mathcal{D}$ denote the space of dynamic output-feedback controllers subject to some constraints and are compatible with $P$. Often, we assume the controllers in $\mathcal{D}$ stabilize $P$, along with some robustness constraint. Let $J\colon\mathcal{D} \to \mathbf{R}$ denote a cost function we wish to minimize over $\mathcal{D}$. For example, $J$ could be LQG or $H_\infty$. 

The next question becomes, how should we parameterize $\mathcal{D}$? Three ideas come to mind: transfer functions, which capture the frequency-domain aspects of the controller; state-space form, which captures the time-domain aspects of the controller; and input-output form, which captures the data-driven aspect. The latter for example is $y_k=\sum_{i=0}^{\infty}h_iu_{k-i}$

When $J$ is time-domain focused, then parameterize $\mathcal{D}$ in state-space form is more adept to gradient-based optimizers. Taking the gradient of LQG with respect to the polynomial coefficients of the transfer function is not realizable. However, we enter an issue. Often, the cost functions depend solely on the input-output properties of the closed loop system. As a result, the coordinates of the internal state of the controller do not matter. That is, if $(A,B,C) \in \mathcal{D}$, then $J(A,B,C)=J(TAT^{-1},TB,CT^{-1})$. This creates redundancy in the search space.

This brings us to a fourth way of parameterize $\mathcal{D}$: quotient spaces. 






\textbf{to do list:}\\
- Collect and decide on the literature on geometry and control, Roger Brockett, Wonham, Kalman, and Robert Hermann.... (notice the gap of these work with the LMI techniques)



-Complete the Permission Log which is available on the
‘Resources’ tab of EMSS. We ask that you complete
the permissions log to identify whether the artwork is
either original, copyright free or copyrighted material.

-Please note that it is the Author’s responsibility to
obtain permission to reproduce any copyrighted
material.


==> geometry-performance.tex <==
\section{Geometry of Performance Objectives on Stabilizing Policies} \label{section:LQ-performance}



In this section, we turn our attention toward performances measures described in \S 2 and the interplay of domain geometry and the landscape of the cost functions associated with each performance measure. Before getting to each specific metric, we review some of the geometric constructs that are essential in characterizing the first and second-order variations of smooth cost functions, subsequently used for optimization.







\subsection{Riemannian Geometry and Policy Optimization}

For the smooth manifold $\stableK$, a vector field $V:\stableK \to T\stableK$ is a mapping that smoothly assigns every $K \in \stableK$ a tangent vector $V_K \in T_K \stableK$. We can alternatively think of a vector fields as a linear mapping on the space of smooth functions over $\stableK$, sending $f:\stableK \to \mathbb{R}$ to $Vf:\stableK \to \mathbb{R}$ as follows: 
\begin{equation}
    Vf(K) := \diff f_K(V_K)
\end{equation} 

In this section, to distinguish tangent vectors from vector fields, we will denote the former with $V_K$ to emphasize that $V_K$ is a tangent vector in $T_K \stableK$. Now, we can define the gradient of $f$ with respect to the Riemannian metric $\tensor{\cdot}{\cdot}{}^\texttt{L}$ on $\stableK$, denoted by $\grad{f}$. In particular, $\grad f$ is the unique vector field satisfying
\begin{equation}\label{eq:grad-def}
    \tensor{V}{\grad f}{}^\texttt{L} = V f,
\end{equation} for all vector fields $V$. 




\lina{Lina's place holder. Will continue from here.} In order to define second-order variations on smooth functions $f$, such as the Riemannian Hessian, we must introduce a notion of directional derivatives on manifolds. This is referred to as the \textit{affine connection} $\nabla$. Let $V,W$ be vector fields on $\stableK$. The construct $\nabla_V W$ is itself a vector field where, intuitively, $(\nabla_V W)_K$ is the directional derivative of $W$ at $K \in \stableK$ along $V_K \in T_K \stableK$. In order to compute $(\nabla_V W)_K$, we only need the direction $V_K$ and the vector field $W$ locally; we do not need all evaluations of $V$. In addition to Riemannian metrics and retractions, affine connections are an additional Riemannian structure. 

Every Riemannian metric uniquely induces a \textit{compatible} affine connection known as the \textit{Levi-Civita connection}. It is the unique affine connection which satisfies
\begin{equation}
    \nabla_U \tensor{V}{W}{} = \tensor{\nabla_U V}{W}{} + \tensor{V}{\nabla_U W}{}
\end{equation} for any vector fields $U,V,W$ of $\stableK$. We will let $\nabla$ and $\overline{\nabla}$ denote the Levi-Civita connections of $\stableK$ under $\langle .,. \rangle^\texttt{L}$ and the Frobenius inner product $\langle V, W\rangle^\texttt{F} := \tr{V^\transpose W}$, respectively. %

Letting $\fX(\stableK)$ denote the family of vector fields on $\stableK$, we can define the Riemannian Hessian of $f$ in two equivalent ways:

\begin{subequations}\label{eq:hess-def}
\begin{align}
    \hess f(V) &:= \nabla_V \grad f \\
    \hess f(V, W) &:= \langle \nabla_V \grad f, W \rangle^\texttt{L}
\end{align}
\end{subequations} Both forms can be used interchangeably. The former is used in the context of Riemannian-Newton optimization. The latter is used in the context of defining a matrix representing the Hessian matrix of $f$. It should be noted that for both definitions, $V,W$ do not have to be tangent vector \textit{fields}; they could simply be tangent vectors. To emphasize our evaluation at a specific $K \in \stableK$, we will write $\hess f |_K $ for both definitions.


As usual, the Euclidean Hessian is equivalently defined as $\overline{\nabla}^2 f(V) := \overline{\nabla}_V \overline{\nabla} f$. 
At last, we also introduce an atypical yet efficient notion known as the pseudo-Euclidean Hessian which essentially ignores the curvature of the manifold in quantifying the second order behavior of a smooth function. It is constructed by applying the \textit{Euclidean affine connection} $\overline{\nabla}$ on the \textit{Riemannian Hessian} $\hess f$ as follows:
\begin{equation}
    \overline{\hess} f(V) := \overline{\nabla}_V \grad f
\end{equation}
which will be compared with the Riemannian Hessian $\hess f$.



\definecolor{myblue}{RGB}{0, 190, 255}
\definecolor{myviolet}{RGB}{126, 47, 142}
\begin{figure}[t]
    \centering
    \begin{overpic}[width=.5\textwidth]{figures/stab_cert_plot.pdf}
        \put(98,85){$K$}
        \put(100,140){\color{red} $V_K$}
        \put(98,105){\color{myviolet} \small $\eta V_K$}
        \put(125,70){\color{myviolet} \scriptsize $\mathcal{B}_K(\eta)$}
        \put(160,120){\color{myblue} $\tilde{\stableK}$}
    \end{overpic}
    \caption{\spencer{thoughts on this?}Illustration of Riemannian gradient descent and the stability certificate in an SLQR problem. We are using the same $\tilde{\stableK}$ as Figure \ref{fig:LQR-simple}. Here, $V_K := - \grad J_\texttt{LQR}(K)$ and $\eta := s_K(V_K)$. Clearly $K + V_K \not \in \tilde{\stableK}$, but we are guaranteed $K + \eta V_K \in \tilde{\stableK}$ since $s_K(\cdot)$ offers a closed-form continuous lower bound on the distance to $\partial \tilde{\stableK}$.}
    \label{fig:stabcert}
\end{figure}




\subsection{Stability Certificate for the Euclidean Retraction}
For the manifold of static feedback policies $\mathcal{S}$, a useful example of a retraction is the Euclidean retraction: $\overline{\mathcal{R}}_K(V_K):= K + V_K$. Note that this is not well-defined globally on $T_K\stableK$, and thus motivates us to further determine the local neighborhood on which it will be well-defined; see \Cref{fig:stabcert}.

\begin{lemma}\label[lemma]{lem:stability-cert}
For any direction $V_K \in T_K\stableK \cong \Kmatrices$ at any point $K \in \stableK$, if 
\begin{equation*}
    0 \leq \eta \leq s_K(V_K) \coloneqq \frac{1}{2 \lambda_{\max}\left(\lyap(A_{\cl}^\transpose, I)\right) \|BV_K\|_2 }
\end{equation*}
where $A_{\cl} = A+BK$, then $K^+ \coloneqq K + \eta V_K \in \stableK$.
\end{lemma}

A few remarks are in order. First, since $\stableK \subset \Kmatrices$ is open, the stability certificate offers a closed-form expression of a continuous lower bound on the radius to instability: $s_K(V_K) \leq \sup \{t:t > 0 , K + tV_K \in \stableK\}$, which has an unknown closed-form expression. In the structured LQR setup, since $\constraint$ is an affine space, $s_K(\cdot)$ is a stability certificate on $\widetilde{\stableK}$ as well. Given $K \in \widetilde{S}$ and $V_K\in T_K \widetilde{\stableK}$, then
\begin{equation}\label{eq:RGD-step}
    K^+ := \overline{\mathcal{R}}_K(\eta V_K) = K + \eta V_K
\end{equation} for $\eta = \min(1, s_K(V_K))$ renders $K^+ \in \widetilde{S}$. Thus for Riemannian gradient descent (\ref{eq:RGD-step}), the chosen step size guarantees feasibility and stability of $K^+ \in \widetilde{S}$. 

For the LQR setup, the direction $V_K$ could the negated Riemannian gradient $-\grad J_\texttt{LQR}(K)$ or Euclidean gradient $-\overline{\nabla} J_\texttt{LQR}(K)$ of the LQR cost. The direction could also incorporate second-order information, in the form of a Riemannian-Newton optimization, formulated as the solution $V_K \in T_K\stableK$ of any of the the linear equations
\begin{align*}
    \hess J_\texttt{LQR} |_K (V) &= -\grad J_\texttt{LQR}(K) \\
    \overline{\nabla}^2 J_\texttt{LQR} |_K(V) &= -  \overline{\nabla} J_\texttt{LQR}(K) \\
    \overline{\hess} J_\texttt{LQR} |_K(V) &= -  \grad J_\texttt{LQR}(K).
\end{align*} Additionally, for structured LQR setup, we show that these first and second order variations can be obtained similarly for the constrained cost $h = J |_{\substableK}$ and the policy update proceeds similarly.
    







\spencer{todo: make this connect with the newly revised section above}
\begin{remark}\label{rem:hewer}
In the absence constraint when $\substableK=\stableK$, the Hewer's algorithm introduces the following updates 
$K^+ = -(B^\transpose P_{K} B + R)^{-1}B^\transpose P_{K
} A,$
which is shown to converge to the global optimum quadratically. Somewhat interestingly, it
in can be written as 
$K^+ = K + \widehat{V},$
with a ``Riemannian quasi-Newton'' direction $\widehat{V}_t$ satisfying,
\[\widehat{H}_{K}\widehat{V} = - \grad{J}_{\texttt{LQR}}(K)\]
where $\widehat{H}_{K}: = (R+B^\transpose P_{K} B)$ is a positive definite approximation of $\hess J_\texttt{LQR}|_K$ and $\overline{\hess} J_\texttt{LQR}|_K$.
The \emph{algebraic coincidence} is that the unit stepsize remains stabilizing throughout these quasi-Newton updates. 
We will also see that for the unconstrained LQR problem a small enough (fixed) step-size is sufficient.
In general though, we do not expect such stepsizes to be stabilizing, and particularly on constrained submanifolds $\substableK$ one needs to instead utilize
the stability certificate developed in \Cref{lem:stability-cert} to guarantee the stability of each policy iterate.
\end{remark}

\subsection{Linear Quadratic Regulator (LQR)}

We here discuss the nonconvex geometry in the policy optimization for LQR. We consider both the standard (unconstrained) case, where the policy parameter $K$ can be a dense matrix, and the constrained case, where $K$ has extra linear constraints in addition to the stabilizing requirement.  

\subsubsection{Unconstrained Case}\label{susec:standard-LQR-perf}

First, by the \lyaptrace~ property in \Cref{lem:dlyap}, one can show that for the static feedback parameterization $u_t = K x_t$ where $K \in \stableK$, both the cost functions in \cref{eq:LQR-noise} and \cref{eq:LQR-noiseless} are equivalent with 
\begin{equation} \label{eq:LQR-cost-lyapunov}
J_{\texttt{LQR}}(K) = \frac{1}{2} \tr{P_K \Sigma} = \frac{1}{2} \tr{(Q+K^\transpose R K) Y_K},
\end{equation}
where $P_K = \lyap(A_{\cl}^\transpose, Q+ K^\transpose R K)$, $Y_K = \lyap(A_{\cl}, \Sigma)$, and $A_{\cl} = A+BK$.
Next, the first and second variations of the smooth cost $J_{\texttt{LQR}} \in C^\infty(\stableK)$ with respect to the Riemannian and Euclidean metrics are obtained in the following proposition.


\begin{proposition}
    Consider the Riemannian manifold $(\stableK, \tensor{.}{.}{}^\texttt{L})$. Then $J_\texttt{LQR}(\cdot)$ is smooth and
    \begin{align*}
        \grad J_\texttt{LQR}(K) &= RK + B^\transpose P_K A_{\cl} \\
        \overline{\nabla} J_\texttt{LQR}(K) &= (RK + B^\transpose P_K A_{\cl}) Y_K,
    \end{align*} where $Y_K = \lyap(A_{\cl}, \Sigma)$. 

    Let $\Gamma_{(k,l),(p,q)}^{(i,j)}$ denote the Christoffel symbols\footnote{See \citep{talebi_policy_2023} for explicit formulas of these smoothly varying scalars that essentially takes the curvature of the manifold into account in computing the Riemannian Hessian.} of $\nabla$ and define 
    \begin{equation}\label{eq:S-map}
        S_K(V_K):= \lyap(A_{\cl}^\transpose, V_K^\transpose \grad J_\texttt{LQR}(K) + (\grad J_\texttt{LQR}(K) )^\transpose V_K).
    \end{equation} Then the Riemannian, Euclidean, and Pseudo-Euclidean Hessians of $J_\texttt{LQR}(\cdot)$ have the following closed-form expressions:
    \begin{subequations}\label{eq:the-hessians}
        \begin{align}
            \hess J_\texttt{LQR} |_K (V_K,W_K) &= \tensor{ B^\transpose S_K(W_K) A_{\cl}}{V_K}{K}^\texttt{L} +\tensor{(R+B^\transpose P_K B) V_K + B^\transpose S_K(V_K)A_{\cl}}{W_K}{K}^\texttt{L} \nonumber\\
            &\quad\textstyle - \tensor{\grad J_\texttt{LQR}(K)}{\sum_{ i,k,p =1}^n \sum_{j,l,q=1}^m [V_K]_{k,l} [W_K]_{p,q}  \Gamma^{i,j}_{(k,l)(p,q)}(K) \partial_{i,j}}{K}^\texttt{L},\nonumber\\
            \overline{\nabla}^2 J_\texttt{LQR} |_K(V_K,W_K) &= \tensor{ B^\transpose S_K(W_K) A_{\cl}}{V_K}{}^\texttt{F} +\tensor{(R+B^\transpose P_K B) V_K + B^\transpose S_K(V_K)A_{\cl}}{W_K}{}^\texttt{F},\nonumber\\
            \overline{\hess} J_\texttt{LQR} |_K(V_K,W_K) &= \tensor{ B^\transpose S_K(W_K) A_{\cl}}{V_K}{K}^\texttt{L} +\tensor{(R+B^\transpose P_K B) V_K + B^\transpose S_K(V_K)A_{\cl}}{W_K}{K}^\texttt{L}.\nonumber
        \end{align}
    \end{subequations} Here, $\partial_{i,j} \in \Kmatrices$ is the matrix with entry $(i,j)$ is set to 1 and all other entries set to 0. 
        
\end{proposition}


Next, we review the properties of this cost function critical to policy optimization.
\begin{lemma}\label[lemma]{lem:coercive}
Suppose $\Sigma, Q, R \succ 0$ and $(A,B)$ is stabilizable. Then, the function $J_{\texttt{LQR}}(\cdot)\colon\mathcal{S} \to \bR$ 
\begin{itemize}
    \item is analytic and
    \begin{equation}
        J_{\texttt{LQR}}(K) = \frac{1}{2}\sum_{t=0}^\infty (A_{\cl}^\transpose)^t (Q + K^\transpose R K) A_{\cl}^t
    \end{equation} is absolutely convergence;
    
    \item is coercive: $K \to \partial \stableK$ or $\|K\|_F \to \infty$ implies $J_\texttt{LQR}(K) \to \infty$;

    \item admits a unique global minimum $K^*$ on $\stableK$ satisfying $K^* = -(R + B^\transpose P_K B)^{-1} B^\transpose P_K A$ where $P_K$ comes from a Riccati equation. %
    
    \item has compact sublevel sets $\stableK_\alpha := \{K:J_\texttt{LQR}(K) \leq \alpha\}$;

    \item is gradient dominant on each sublevel set: there exists a constant $c_1 >0$ such that
    \[c_1 [J_{\texttt{LQR}}(K)-J_{\texttt{LQR}}(K^*)] \leq  \| \overline{\nabla} J_{\texttt{LQR}}(K) \|_F^2, \quad \forall K \in \stableK_\alpha;\]

    \item is $L$-Lipchitz on each sublevel set: there exists a constant $L>0$ such that
    \[\|\overline{\nabla} J_{\texttt{LQR}}(K) - \overline{\nabla} J_{\texttt{LQR}}(K')\|_F \leq L  \|K - K'\|_F, \quad \forall K,K' \in \stableK_\alpha;\]

    \item  admits lower and upper quadratic models on each sublevel set: there exists constants $c_2 >0$ and $c_3 >0$ such that
    \[c_2 \|K-K^*\|^2_F \leq  J_{\texttt{LQR}}(K)-J_{\texttt{LQR}}(K^*) \leq c_3 \|K-K^*\|^2_F, \quad \forall K \in \stableK_\alpha.\]
\end{itemize}
\end{lemma}

These properties of $J_\texttt{LQR}$ are quite essential in providing theoretical guarantees for different optimization schemes. In particular, the smoothness, Lipschitz continuity, and quadratic models are common in convex optimization whereas the gradient dominance enables global convergence guarantees despite non-convexity of $J_{\texttt{LQR}}$ in $K$. Finally, note that these properties holds on each (fixed) sublevel set of the cost which often is chosen to contain the initial policy $K_0$. These has made possible due to the coercive property of $J_{\texttt{LQR}}$ that results in compact sublevel sets. 



\subsubsection{Linearly Constrained case}\label{sec:lin-constrained-policy-performance}

Here, we will discuss the Riemannian geometry of the LQR cost in the structured LQR setup. Since $\widetilde{\stableK} := \stableK \cap \constraint \subset \stableK$ is an embedded submanifold, the Riemannian metric $\langle .,. \rangle^\texttt{L}$ can be equipped onto $\widetilde{\stableK}$ simply by restricting its domain $T\stableK$ onto $T\widetilde{\stableK}$. For any smooth function $f$ on $\stableK$, let $\widetilde{f}:=f|_{\widetilde{\stableK}}$ be its restriction.

First note that the restriction of $\grad f$ to $\widetilde{\stableK}$ is not a well-defined vector field due to the possibility of $\grad f(K) \not \in T_K \widetilde{\stableK}$. It follows to ask what is the Riemannian gradient of $\widetilde{f}$, denoted as $\grad \widetilde{f} : \widetilde{\stableK} \to T \widetilde{\stableK}$. 


Let $K \in \widetilde{\stableK}$. Define $N_K \widetilde{\stableK} := \{V_K \in T_K \stableK: \langle V_K, W_K \rangle_K^\texttt{L} = 0 \ \forall W_K \in T_K \widetilde{\stableK}\}$. It is easy to see there exists a unique $V_K^\top \in T_K \widetilde{\stableK}$ and $V_K^\perp \in N_K \widetilde{\stableK}$ in which $V_K = V_K^\top + V_K^\perp$. Furthermore, we will always have $V_K^\perp = V_K - V_K^\top$. This induces the well-defined operators on vector fields: $\pi^\top(V):=V^\top$ and $\pi^\perp(V) := V^\perp$ are called the Riemannian tangential and normal projections. \shahriar{I think the language can be improved by having smooth sentences.}

Recall the Levi-Civita connection $\nabla$ uniquely induced from $\langle .,. \rangle^\texttt{L}$. Using the tangential projection, we can determine the Levi-Civita connection on $\widetilde{\stableK}$ induced from the Riemannian metric restricted onto $\widetilde{\stableK}$ as follows. Let $V, W \in \fX(\widetilde{\stableK})$. Then
\begin{equation}
    \widetilde{\nabla}_V W := \pi^\top \nabla_V W.
\end{equation} Now that we have the Levi-Civita connection, we may define the Riemannian gradient $\grad \widetilde{f}$ as we did in (\ref{eq:grad-def}) and (\ref{eq:hess-def}).

For second-order variations, i.e. computing $\hess \widetilde{f}$, we need the following geometric construct that captures the effect of the curvature in second-order derivatives. Let $V \in \fX(\widetilde{\stableK})$ and let $U \in \fX(\stableK)$ be a \textit{normal vector field} satisfying $U_K \in N_K \widetilde{\stableK}$ for all $K \in \widetilde{\stableK}$. Define the \textit{Weingarten map} $\mathbb{W}_U(V) \in \fX(\widetilde{\stableK})$ as the unique solution to
\begin{equation}
    \langle \mathbb{W}_U(V), W \rangle^\texttt{L} = \langle U, \pi^\perp \nabla_V W \rangle^\texttt{L}
\end{equation} for all $W \in \fX(\widetilde{\stableK})$. 

\begin{proposition}
    Let $f:\stableK \to \mathbb{R}$ and $\widetilde{f}:=f|_{\widetilde{\stableK}}$. Then over $\widetilde{\stableK}$, we have
    \begin{equation}
        \grad \widetilde{f} = \pi^\top \grad f.
    \end{equation} Furthermore, for any $V \in \fX(\widetilde{\stableK})$, we have
    \begin{equation}
        \hess \widetilde{f}(V) = \pi^\top \hess f(V) + \mathbb{W}_U (V),
    \end{equation} where $U := \pi^\perp \grad f$. 
\end{proposition}

This result enables us to obtain explicit formulae for the Riemannian gradient and hessian of any smooth costs on $\stableK$ when restricted to $\widetilde{\stableK} = \stableK \cap \constraint$. In fact, this is proved for any embedded submanifold of an abstract Riemannian manifold.  As expected, these geometric derivatives will be affected by the curvature of $(\stableK, \langle .,. \rangle^\texttt{L})$ which is accurately captured by the second term of the Weingarten mapping. In explicit form, these can be computed using the Christoffel symbols associated with induced Levi-Civita connection $\nabla$; see \cite[Prop. 3.4]{talebi_policy_2023} for the general proof and explicit formulae of these quantities.

By direct application of these results to the constraint LQR cost $\widetilde{J}_\texttt{LQR} := J_\texttt{LQR}|_{\widetilde{\stableK}}$, we can give explicit formulae for Riemannian gradient and Hessian:
\begin{align*}
    \grad \widetilde{J}_\texttt{LQR}(K) &= \pi^\top (RK + B^\transpose P_K A_{\cl}) \\
    \overline{\nabla} \widetilde{J}_\texttt{LQR}(K) &= \text{Proj}_K((RK + B^\transpose P_K A_{\cl})Y_K),
\end{align*} where $\text{Proj}_K$ is the ordinary Euclidean projection operator from $T_K \stableK$ onto $T_K \widetilde{\stableK}$.
Also, similarly for the Riemannian, Euclidean, and Pseudo-Euclidean Hessians for $\widetilde{J}_\texttt{LQR}(\cdot)$ are
\begin{align*}
    \hess \widetilde{J}_\texttt{LQR} |_K (V_K,W_K) &= \tensor{ B^\transpose S_K(W_K) A_{\cl}}{V_K}{K}^\texttt{L} +\tensor{(R+B^\transpose P_K B) V_K + B^\transpose S_K(V_K)A_{\cl}}{W_K}{K}^\texttt{L} \\
    &\textstyle - \tensor{\grad J_\texttt{LQR}(K)}{\sum_{ i,k,p =1}^n \sum_{j,l,q=1}^m [V_K]_{k,l} [W_K]_{p,q}  \Gamma^{i,j}_{(k,l)(p,q)}(K) \partial_{i,j}}{K}^\texttt{L},\\
    \overline{\nabla}^2 \widetilde{J}_\texttt{LQR} |_K(V_K,W_K) &= \tensor{ B^\transpose S_K(W_K) A_{\cl}}{V_K}{}^\texttt{F}
      +\tensor{(R+B^\transpose P_K B) V_K + B^\transpose S_K(V_K)A_{\cl}}{W_K}{}^\texttt{F},\\
     \overline{\hess} \widetilde{J}_\texttt{LQR} |_K(V_K,W_K) &= \tensor{ B^\transpose S_K(W_K) A_{\cl}}{V_K}{K}^\texttt{L}
     +\tensor{(R+B^\transpose P_K B) V_K + B^\transpose S_K(V_K)A_{\cl}}{W_K}{K}^\texttt{L}.
    \end{align*} where $\Gamma^{i,j}_{(k,l)(p,q)}(K)$ is the Christoffel symbol of $\nabla$ and $S_K(\cdot)$ is defined in (\ref{eq:S-map}). 

Finally in \Cref{fig:LQR-landscape-constrained}, we provide a numerical illustration of how this Riemannian metric is useful, and how the curvature information is enabling us to obtain better directions of descent and more effective algorithms. We are simulating the same example as in \Cref{fig:SLQR-landscape} where the controller is constrained to be diagonal.



\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width = 0.46\textwidth]{figures/slqr_landscape.pdf}}
    \subfigure[]{ \includegraphics[width = 0.52\textwidth]{figures/NewtonGD_slqr.eps}}
    \caption{A numerical example for the feasible set of diagonal stabilizing controller for the \ac{slqr} problem of \S 2. a) the region on which the Riemannian Hessian is positive definite versus that of Pseudo-Euclidean Hessian. (b) Trajectories of the QRNPO algorithm \citep{talebi_riemannian_2022} using Riemannian Hessian in blue, incorporating the curvature, versus the Euclidean Hessian in orange.\spencer{could we increase the font size}\shahriar{Is this better for now?}\spencer{idk if im seeing things but the fonts do not seem consistent between left and right images}}
    \label{fig:LQR-landscape-constrained}
\end{figure}







\subsection{Linear Quadratic Gaussian (LQG) control}\label{subsec:LQG}

In this subsection, we move to discuss the geometry in policy optimization for LQG control \eqref{eq:LQG_policy-optimization}. As we will see below, while sharing certain similarities, the non-convex LQG landscape is richer and more complicated than the LQR case. 


Recall that the set of stabilizing policies $\mathcal{C}_n$  has at most two path-connected components that are diffeomorphic to each other under a particular similarity transformation (\Cref{Theo:disconnectivity}). As similarity transformations do not change the input/output behavior of dynamic policies, it makes no difference to search over any path-connected component even if $\mathcal{C}_n$ is not path-connected. This feature brings positive news for local policy search algorithms over dynamic stabilizing policies $\mathcal{C}_n$. %


\subsubsection{Spurious Stationary Points and Global Optimality}

Similar to the LQR case, for any stabilizing policy $\mK\in\mathcal{C}_n$, the LQG cost function $J_{\texttt{LQG}}(\mK)$ in \eqref{eq:LQG_policy-optimization} has the following expression: 
\begin{equation}\label{eq:LQG_cost_formulation_discrete}
J_{\texttt{LQG}}(\mK) = \operatorname{tr}
\left(
\begin{bmatrix}
Q & 0 \\ 0 & C_{\mK}^\transpose R C_{\mK}
\end{bmatrix} X_\mK\right)
=
\operatorname{tr}
\left(
\begin{bmatrix}
W & 0 \\ 0 & B_{\mK} V B_{\mK}^\transpose
\end{bmatrix} Y_\mK\right),
\end{equation}
where $X_{\mK}$ and $Y_{\mK}$ are the unique positive semidefinite 
solutions to the Lyapunov equations below 
\vspace{-1mm}
\begin{subequations}
\begin{align}
X_{\mK} &= \begin{bmatrix} A &  BC_{\mK} \\ B_{\mK} C & A_{\mK} \end{bmatrix}X_{\mK}\begin{bmatrix} A &  BC_{\mK} \\ B_{\mK} C & A_{\mK} \end{bmatrix}^\transpose +  \begin{bmatrix} W & 0 \\ 0 & B_{\mK}VB_{\mK}^\transpose  \end{bmatrix}, \label{eq:LyapunovX_discrete}
\\
Y_{\mK} &= \begin{bmatrix} A &  BC_{\mK} \\ B_{\mK} C & A_{\mK} \end{bmatrix}^\transpose Y_{\mK}\begin{bmatrix} A &  BC_{\mK} \\ B_{\mK} C & A_{\mK} \end{bmatrix} +   \begin{bmatrix} Q & 0 \\ 0 & C_{\mK}^\transpose R C_{\mK} \end{bmatrix}. \label{eq:LyapunovY_discrete}
\end{align}
\end{subequations}
Note that $X_{\mK}$ and $Y_{\mK}$ are closely related to the controllable and observable Gramians of the closed-loop system \eqref{eq:closed_loop_system}. 

From \eqref{eq:LQG_cost_formulation_discrete}, it is not difficult to see that $J_{\texttt{LQG}}(\mK)$ is a rational function in terms of the policy parameter $\mK$, and it is thus a real analytic function on $\mathcal{C}_n$. We summarize this as a fact below.%
\begin{fact}
    The LQG cost $J_{\texttt{LQG}}(\mK)$ in \eqref{eq:LQG_policy-optimization}  is real analytic on $\mathcal{C}_n$, and in particular smooth. 
\end{fact}


\begin{figure}[t]
\centering
    \includegraphics[width = 0.35\textwidth]{figures/LQG_unstable.eps}
    \hspace{15mm}
\includegraphics[width=0.35\textwidth]{figures/LQG_stable.eps}

    \caption{Non-isolated and disconnected optimal LQG policies (highlighted by the red curves). In both cases, we set $Q = 1$, $R = 1, V = 1, W = 1 $. (a) LQG cost for the open-loop unstable system with $A=1.1, B = C =1$, where we fixed $A_\mK = -0.3069$; (b) another LQG cost for the open-loop stable system with $A=0.9, B = C =1$, where we fixed $A_\mK = -0.1753$. In the right subfigure, the origin $B_\mK = 0, C_\mK = 0$ with $A_{\mK} = -0.1753$ is a saddle point.}
    \label{fig:LQG-shape}
\end{figure}


It is also easy to identify examples to confirm the nonconvexity of LQG policy optimization \eqref{eq:LQG_policy-optimization} (note that the domain $\mathcal{C}_n$ is already nonconvex; see \Cref{fig:feasible_region}). Unlike the LQR, it is known that the problem of LQG problem \eqref{eq:LQG_policy-optimization} has non-unique and non-isolated globally optimal policies in the state-space form $\mathcal{C}_n$. This is not difficult to see since any similarity transformation on one optimal LQG policy $\mK^\star$ leads to another optimal solution that achieves the same cost, i.e., 
\begin{equation} \label{eq:similarity-transformation-LQG}
J_{\texttt{LQG}}(\mK^\star) = J_{\texttt{LQG}}(\mathscr{T}_T(\mK^\star)), \quad \forall T \in \mathrm{GL}_n.
\end{equation}
\Cref{fig:LQG-shape} illustrates the non-convex LQG landscape and the non-isolated/disconnected optimal LQG policies. It is also known that the LQG cost  $J_{\texttt{LQG}}$ is not coercive: there might exist sequences of stabilizing policies $\mK_j \in \mathcal{C}_n$ where $\lim_{j \rightarrow \infty} \mK_j \in \partial \mathcal{C}_n$ such that 
$
    \lim_{j \rightarrow \infty} J_{\texttt{LQG}}(\mK_j) < \infty,  
$
and sequences of stabilizing policies $\mK_j \in \mathcal{C}_n$ where $\lim_{j \rightarrow \infty} \|\mK_j\|_F = \infty$ such that 
$
    \lim_{j \rightarrow \infty} J_{\texttt{LQG}}(\mK_j) < \infty. 
$
The latter fact is easy to see from the effect of similarity transformation \eqref{eq:similarity-transformation-LQG} since $J_{\texttt{LQG}}(\mK)$ is constant for policies that are connected by any $T \in \mathrm{GL}_n$; also see \cite[Example 4.1]{zheng2023benign} for the former fact.
The following lemma gives a closed-form expression for the gradient of the LQG cost function $J_{\texttt{LQG}}$.


\begin{lemma} \label[lemma]{lemma:gradient_LQG_Jn_discrete}
   The (standard) gradient of $J_{\texttt{LQG}}$ at $\mK = (A_\mK, B_\mK, C_\mK) \in \mathcal{C}_n$ is given by
    \begin{subequations} \label{eq:gradient_Jn_discrete}
        \begin{align}
         \frac{\partial J_{\texttt{LQG}}(\mK)}{\partial A_{\mK}} &= 2\left(Y_{12}^\transpose(AX_{12}+BC_{\mK}X_{22}) + Y_{22}A_{\mK}X_{22} + Y_{22}B_{\mK}CX_{12}\right), \label{eq:partial_Ak_discrete}\\
        \frac{\partial J_{\texttt{LQG}}(\mK)}{\partial B_{\mK}} &= 2\left(Y_{12}^\transpose(AX_{11} + BC_{\mK}X_{12}^\transpose)C^\transpose +  Y_{22} A_{\mK} X_{12}^\transpose C^\transpose +  Y_{22}B_{\mK}(CX_{11}C^\transpose+V)\right), \label{eq:partial_Bk_discrete}\\
        \frac{\partial J_{\texttt{LQG}}(\mK)}{\partial C_{\mK}} &= 2\left(B^\transpose Y_{12}(A_{\mK}X_{22} + B_{\mK} CX_{12}) + B^\transpose Y_{11}AX_{12} + (B^\transpose Y_{11}B + R)C_{\mK}X_{22}\right), \label{eq:partial_Ck_discrete}
        \end{align}
    \end{subequations}
    where $X_{\mK}$ and $Y_{\mK}$, partitioned as 
     $   X_{\mK} = \begin{bmatrix}
        X_{11} & X_{12} \\ X_{12}^\transpose & X_{22}
        \end{bmatrix},  \; Y_{\mK} = \begin{bmatrix}
        Y_{11} & Y_{12} \\ Y_{12}^\transpose & Y_{22}
        \end{bmatrix}$
    are the unique positive semidefinite 
    solutions to~\eqref{eq:LyapunovX_discrete} and~\eqref{eq:LyapunovY_discrete}, respectively.
\end{lemma}

As shown in \Cref{fig:LQG-shape}, the set of stationary points $\{\mK \in \mathcal{C}_n \mid \nabla J_{\texttt{LQG}}(\mK) = 0\}$ is not isolated and can be disconnected. Furthermore, there may exist strictly suboptimal spurious stationary points for the LQG control \eqref{eq:LQG_policy-optimization}. This fact can be seen from the right figure of \Cref{fig:LQG-shape}, in which the policy $\mK \in \mathcal{C}_1$ with values $A_\mK =   -0.1753$, $B_\mK = 0$, and $C_\mK = 0$ corresponds to a saddle point.  
Indeed, the following result explicitly characterizes a class of saddle points in LQG control \eqref{eq:LQG_policy-optimization} when the plant dynamics are open-loop stable. These stationary points are spurious and suboptimal whenever the globally  optimal LQG policy corresponds to a nonzero transfer function.  



\begin{theorem}[Saddle points in LQG] \label{theorem:saddle}
    Suppose \eqref{eq:dynamics_discrete} is open-loop stable. Let $A_\mK = \Lambda\in\mathbb{R}^{n\times n}$ be any stable matrix. Then the zero policy $\mK \in \mathcal{C}_n$ with parameters $A_\mK = \Lambda, B_\mK = 0, C_\mK = 0$ is a stationary point of $J_{\texttt{LQG}}(\mK)$ over $\mathcal{C}_n$, and the corresponding Hessian is either indefinite or zero.
\end{theorem}

Due to the existence of spurious saddle points, LQG policy optimization \eqref{eq:LQG_policy-optimization} cannot enjoy the gradient dominance property as the LQR case. The gradient dominance property will also fail for the LQG control even when an observed-based policy parameterization is used \citep{mohammadi2021lack}. Note that the policy $\mK$ in \Cref{theorem:saddle} corresponds to a zero transfer function, and the policy just produces a zero input. It has been shown that \textit{all spurious stationary points $\mK$ are none-minimal dynamic policies}, i.e., either $(A_\mK, B_\mK)$ is not controllable, or $(C_\mK, A_\mK)$ is not observable or both. Therefore, we have the following result about globally optimal LQG policies.    

\begin{theorem}[Global optimality in LQG]\label{thm:global-optimum}
    All stationary points that correspond to controllable and observable policies are globally optimal in the LQG problem \eqref{eq:LQG_policy-optimization}. These globally optimal policies are related to each other by a similarity transformation. 
\end{theorem}

The proof is based on closed-form gradient expressions for controllable and observable stationary points $\mK \in \mathcal{C}_n$ (by letting the gradients in \eqref{eq:gradient_Jn_discrete} equal to zero), which are shown to be same as the optimal solution from Riccati equations. This proof strategy was first used in \citep{hyland1984optimal} to derive first-order necessary conditions for optimal reduced-order controllers. It strongly depends on the assumption of minimality, which fails to deal with non-minimal globally optimal policies for LQG control. Beyond minimal policies, a recent extension of global optimality characterization in LQG control is \cite[Theorem 4.2]{zheng2023benign}, which is based on a notion of \textit{non-degenerate} stabilizing policies. This characterization relies on a more general strategy~of~extended convex lifting that captures a suitable convex re-parameterization of LQG control~\eqref{eq:LQG_policy-optimization}.  







\subsubsection{Invariances of LQG: a Quotient Geometry} \label{subsection:symmetry-manifold-structures-LQG}
This subsection is a sequel to the quotient manifold setup introduced in \S\ref{subsubsec:invariants_of_feedback_policies}. Recall the LQG cost $J_{\texttt{LQG}}$ solely depends on the input-output properties of the closed loop system. If our parameterization of choice is the state-space form in (\ref{eq:internallystabilizing}), then the control design objective will be invariant under similarity transformation (\ref{eq:def_sim_transform}): 
\begin{equation*}
    J_{\texttt{LQG}}(\mK) = J_{\texttt{LQG}}(\mathscr{T}_T(\mK)) \ \forall \mK \in \mathcal{C}_n, \forall T \in \mathrm{GL}_q.
\end{equation*} Figure \ref{fig:LQG_cost_on_manifold_and_orbits} shows the LQG cost on $\mathcal{C}_1$.

\begin{figure}[t]
    \centering
    \includegraphics[width = .4\textwidth]{./figures/dynamic_controller_LQG_cost.pdf}
    \caption{A colored plot of the LQG cost $J_\texttt{LQG}(\cdot)$ over $\mathcal{C}_n$ with $A=1.1, B = C = 1$. Color is determined via an affine transformation of $\log(J_\texttt{LQG}(\mK))$ so that the minimum LQG cost is mapped to 0 and the maximum LQG cost is mapped to 1, over the given plot bounds on $A_\mK, B_{\mK}, C_{\mK}$.}
    \label{fig:LQG_cost_on_manifold_and_orbits}
\end{figure}

The similarity-invariance of LQG causes many hindrances for policy optimization. First, each stationary point lies within an orbit of stationary points, and this orbit will have dimension $n^2$. Therefore, the Hessian of any stationary point will be non-singular: its nullspace dimension will be at least $n^2$. This slows the convergence rate of policy optimization algorithms. Also, local convergence guarantees will be more difficult to obtain since the Hessian at the global minimum cannot be positive-definite. 

Second, since the dot product is not coordinate-invariant, we loose the useful invariance property:
\begin{equation*}
    \overline{\nabla} J_{\texttt{LQG}} ( \mathscr{T}_T(\mK))  \not = \mathscr{T}_T(\overline{\nabla} J_{\texttt{LQG}} (\mK)).
\end{equation*} This has impacts on the initialization; if we choose a particularly bad initialization $\|K_0\|_F >> 1$, then we will always have $\|\overline{\nabla} J_{\texttt{LQG}}(\mK) \|_F >> 1$. This also implies that gradient descent fails to satisfy the following property known as similarity-equivariance:
\begin{equation}\label{eq:sim-equivariance}
    \mathscr{T}_T(\mK - \alpha \overline{\nabla} J_{\texttt{LQG}}(\mK)) \not = \mathscr{T}_T(\mK) - \alpha \overline{\nabla} J_{\texttt{LQG}}(\mathscr{T}_T(\mK)).
\end{equation} As we will see, we can resolve these issues by introducing a similarity-invariant Riemannian metric and devising a Riemannian gradient descent procedure. 



Since $J_\texttt{LQG}(\cdot)$ is similarity-invariant, we can induce a unique cost onto the smooth quotient space $\mathcal{C}_n/\mathrm{GL}_n$ as follows:

\begin{equation*}
    \widetilde{J}_{\texttt{LQG}}([\mK]) := J_{\texttt{LQG}}(\mK')
\end{equation*} where $\mK'$ is any controller $\mK' \sim \mK$. Now let us equip $\mathcal{C}_n^{\min}$ with the KM metric (\ref{eq:KM-metric}) and $\mathcal{C}_n^{\min}/\mathrm{GL}_n$ with the corresponding quotient metric. Then the Riemannian gradient is similarity-equivariant (\ref{eq:sim-equivariance}):
\begin{equation*}
    \grad J_\texttt{LQG}(\mathscr{T}_T(\mK)) = \mathscr{T}_T(\grad J_\texttt{LQG}(\mK))
\end{equation*} Using the Euclidean retraction, which is similarity-equivariant, we therefore have the fact that a single step of Riemannian gradient descent is similarity equivariant. That is,
\begin{equation*}
    \mathscr{T}_T(\mK - \alpha \grad J_\texttt{LQG}(\mK)) = \mathscr{T}_T(\mK) - \alpha \grad J_\texttt{LQG}(\mathscr{T}_T(\mK)).
\end{equation*} This is a remarkable property. If we perform a similarity transformation on the initial controller $\mK_0$, giving us $\mK_0' \sim \mK_0$, then the resulting sequence of iterates will also be transformed by that same similarity transformation.

This also implies the following. Let $\mK \in \mathcal{C}_n^{\min}$ and $\mK^+ := \mK - \alpha -\grad J_\texttt{LQG}(\mK)$. Let $\kappa := [\mK] \in \mathcal{C}_n^{\min}/\mathrm{GL}_n$ and define $\chi^+ := \mathcal{R}_{\kappa}(-\alpha \grad \widetilde{J}_\texttt{LQG}(\kappa)$. Then $\chi^+ = [\mK^+]$. In other words, Riemannian gradient descent over the Riemannian quotient manifold coincides with Riemannian gradient descent over the total manifold. We emphasize that these properties hold only when the Riemannian metric is
similarity-invariant (\ref{eq:metric-inv}), such as the KM metric, and the retraction is similarity-equivariant (\ref{eq:retraction-inv}), such as the Euclidean retraction.



We will end this section with a lemma that shows how this setup reduces the nullspace dimension of stationary points. The following result that quantifies the number of eigenvalues of the Riemannian Hessian with positive, zero, and negative signs---referred to as its ``signature''.

\begin{lemma}\label[lemma]{lem:signature}
    Let $\mathcal{M}$ be a manifold under group action $G$ equipped with a $G$-invariant Riemannian metric. Suppose $\mathcal{M}/G$ is a smooth quotient manifold and consider any $G$-invariant function $f:\mathcal{M} \to \mathbb{R}$. If  $(n_-,n_0,n_+)$ is the signature of $\hess f(x^*)$ at any stationary point $x^* \in \mathcal{M}$ of $f$, then the signature of $\hess \widetilde{f}([x^*])$ is $(n_-,n_0-\dim(G),n_+)$, where $\widetilde{f}([x]):=f(x)$.
\end{lemma}
To illustrate a consequence of this lemma, suppose $\mK^*$ is a global minimum of $J_{\texttt{LQG}}$. This implies $\overline{\nabla}^2 J_{\texttt{LQG}}(\mK^*)$ has at least $q^2$ zeros. Due to the lack of positive-definiteness of the Hessian, we are not guaranteed a linear rate of convergence. But, by the above lemma, we can show that $\hess \widetilde{J}_{\texttt{LQG}}([\mK^*])$ has $q^2$ less zeros. This implies that if $\dim \ker \overline{\nabla}^2 J_{\texttt{LQG}}(\mK^*) = q^2$, then $\hess \widetilde{J}_{\texttt{LQG}}([\mK^*]) > 0$. This property is what allowed for a local linear rate of convergence guaranteed in \cite[Thm. 5.2]{kraisler2024output} for the continuous system dynamics. 




\shahriar{Can we add the Riemanninan Hessian and Gradient of LQG under KM metric here?} \spencer{there are no closed-form expressions, i computed them the hard way using local coordinates} \shahriar{That is fine, include some information about what needs to be done.}

\shahriar{Also, please add the final form of the iterative updates for the specific LQG manifold here.}


\subsection{$\mathcal{H}_\infty$-norm: Systems with Adversarial Noises}

In this section, we return to the state-feedback $\mathcal{H}_\infty$ optimal control problem introduced in \S\ref{subsubsect:state-feedback-robust-control}. 
Setting the initial state $x_0 \equiv 0$, then with a stabilizing policy $K \in \mathcal{S}$, the performance $J_\infty(\cdot)$ \eqref{eq:robust-cost} equals the square of the $\mathcal{H}_\infty$ norm of the closed-loop transfer function from $w_t$ to a performance measure 
$
z_t := \begin{bmatrix}
    (Q^{1/2} x_t)^\transpose & (R^{1/2} u_t)^\transpose
\end{bmatrix}^\transpose.\
$
With this, we can equivalently write (\ref{eq:robust-cost}) as
\begin{equation} \label{eq:closed-loop-hinf-norm}
\begin{aligned}
    J_\infty(K) &= \sup_{\|w\|_{l_2} \neq 0} \frac{\|z\|_{l_2}^2}{\|w\|_{l_2}^2}= \left\|\begin{bmatrix}
    Q^{1/2} \\ R^{1/2}K
\end{bmatrix} (zI - A - BK)^{-1}\right\|_\infty^2 \\
&= \sup_{\omega \in [0, 2\pi]}\, \lambda_{\max}\left( (e^{-j\omega} -A - BK)^{-\transpose} (Q + K^\transpose R K) (e^{j\omega} -A - BK)^{-1}\right), 
\end{aligned}
\end{equation}
where $\lambda_{\max}(\cdot)$ denotes the maximal eigenvalue of an Hermitian matrix. %




Unlike the case of LQR or LQG, we usually do not have a closed-form expression to evaluate the $\mathcal{H}_\infty$ norm \eqref{eq:closed-loop-hinf-norm}. One can also use the celebrated KYP lemma to evaluate  it using a linear matrix inequality (LMI), but the solution can take more computational efforts than the counterpart in LQR \eqref{eq:LQR-cost-lyapunov} or LQG \eqref{eq:LQG_cost_formulation_discrete} that only involves solving (linear) Lyapunov equations. %
Classical control techniques typically re-parameterize the nonconvex $\mathcal{H}_\infty$ control \eqref{eq:Hinf-policy-optimization} into a convex LMI via a change of variables \citep{boyd1994linear}, or directly characterize a suboptimal solution via solving a single (quadratic) Riccati equation \citep{zhou1988algebraic}. We here dsicuss some geometrical aspects of the $\mathcal{H}_\infty$ policy optimization \eqref{eq:Hinf-policy-optimization}.   

\begin{figure}
    \centering
    \includegraphics[width = 0.25\textwidth]{figures/Hinf_a.eps}
    \hspace{15mm}
\includegraphics[width=0.33\textwidth]{figures/Hinf_b.eps}
    \caption{Nonconvexity and non-smoothness of the $\mathcal{H}_\infty$ cost function (the problem setup is taken from \cite[Example 5.1]{zheng2023benign}): The left figure illustrates a static output feedback $\mathcal{H}_\infty$ control instance with $u_t = D_{\mK}y_t$ which shows one non-smooth point (highlighted by the black point); the right figure corresponds to a dynamic $\mathcal{H}_\infty$ control instance which exhibits a set of nonsmooth points (highlighted by the red lines). }
    \label{fig:Hinf-landscape} 
\end{figure}

Compared with the cases of LQR and LQG, one major difference in $\mathcal{H}_\infty$ control is that the function $J_{\infty}(K)$ in \eqref{eq:closed-loop-hinf-norm} is non-smooth, i.e., the cost function $J_{\infty}(K)$ may not be differentiable at some feasible points $K \in \mathcal{S}$ (see \Cref{fig:Hinf-landscape} for illustration). This fact is actually not difficult to see due to two possible sources of non-smoothness in \eqref{eq:closed-loop-hinf-norm}: One from taking the largest eigenvalue of complex matrices, and the other from maximization over  $\omega \in [0,2\pi]$. Indeed, robust control problems were one of the early motivations and applications for non-smooth optimization \citep{lewis2007nonsmooth}. Despite the non-smoothness, the $\mathcal{H}_\infty$ cost function is \textit{locally Lipschitz} and thus differentiable almost everywhere (\Cref{fig:Hinf-landscape} also illustrates this). Thus, we can define the Clarke directional derivative and Clarke subdifferential of $J_{\infty}(K)$ at each feasible policy $K \in \mathcal{S}$.  

Furthermore, the $\mathcal{H}_\infty$ cost function $J_{\infty}(K)$ is known to be ``subdifferentially regular'' in the sense of Clarke \citep{clarke1990optimization} (i.e., the ordinary directional derivative exists and coincides with the Clarke directional derivative for all directions).  
Also, it is known that the discrete-time state-feedback $\mathcal{H}_\infty$ cost function \cref{eq:closed-loop-hinf-norm} is coercive.
We summarize these properties property below, which to some extend are analogous to those of LQR cost in \Cref{lem:coercive}.

\begin{lemma}\label[lemma]{lemma:H_inf_some_local_Lipschitz}
Suppose $Q \succ 0, R \succ 0$ and $(A,B)$ is stabilizable. Then, the $\mathcal{H}_\infty$ cost function $J_{\infty}\colon \stableK \mapsto \mathbb{R}$, defined in \eqref{eq:closed-loop-hinf-norm} 
\begin{itemize}
    \item is locally Lipschitz, and thus almost everywhere differentiable;
    
    \item is subdifferentially regular over the set of stabilizing policies $\mathcal{S}$;
    
    \item is coercive\footnote{We remark that this coerciveness property fails to hold in the continuous-time state-feedback $\mathcal{H}_\infty$ control, even when $Q \succ 0, R \succ 0$; see \cite[Fact 4.1]{zheng2024benign}}: $K \to \partial\mathcal{S} \text{ or } \|K\| \to \infty \;\text{ each implies }\; J_{\infty}(K) \to \infty$;
 
    \item has compact, path-connected sublevel sets $\mathcal{S}_\gamma = \{K \in \mathcal{S} \mid J_{\infty}(K) \leq \gamma\}$
    for any $\gamma \geq \gamma^\star : = \min_{K} J_{\infty}(K)$.
     
\end{itemize}
\end{lemma}
  
The proof idea for the first two properties is to view $J_{\infty}(K)$ as a composition of a convex mapping $\|\cdot\|_\infty$ and the mapping from  $K$ to a stable closed-loop transfer function that is continuously differentiable over $\mathcal{S}$. 
In the discrete time, the coerciveness of $J_\infty$ can be proved using the positive definitness of $Q$ and $R$.  
The compactness of sublevel sets follows directly by coercivity. The sublevel set $\mathcal{S}_\gamma$ is in general non-convex but always path-connected, the proof of which is essentially the same as that in \eqref{eq:convexPL}. One can also compute the set of subdifferential  $\partial J_{\infty}(K)$ at each feasible policy $K \in \mathcal{S}$; however, the computation is much more complicated than the smooth LQR or LQG case. We refer the interested reader to \cite[Lemma 5.2]{zheng2023benign} and \cite{apkarian2006nonsmooth} for more details. %
Despite the nonconvex and non-smoothness, we have a global optimality characterization for \eqref{eq:Hinf-policy-optimization}. 

\begin{theorem}[Global optimality in $\mathcal{H}_\infty$ control] \label{theorem:hinf-global-optimality}
    Consider the state-feedback $\mathcal{H}_\infty$ control \eqref{eq:Hinf-policy-optimization} with $Q \succ 0, R \succ 0$. Any Clarke stationary point is globally optimal.  
\end{theorem}

The high-level proof idea of this result is also similar to the change of variables in \eqref{eq:convexPL}: it is known that \eqref{eq:Hinf-policy-optimization} admits an equivalent convex reformulation by a change of variables, and this change of variables can be designed as a diffeomorphism between nonconvex policy optimization and its convex reformulation; this diffeomorphism then allows us to certify global optimality in original non-smooth and nonconvex $\mathcal{H}_\infty$ control. This idea has recently been characterized into a new framework of extended convex lifting (ECL) in \citep{zheng2023benign,zheng2024benign}. In particular,  
let us define its epigraph for the state-feedback $\mathcal{H}_\infty$ control \eqref{eq:Hinf-policy-optimization} as 
$$
\mathrm{epi}_{\geq}(J_\infty) := \{(K,\gamma) \mid J_\infty(K) \leq \gamma, K \in \mathcal{S}\}. 
$$
It is known from classical control theory that $(K,\gamma) \in \mathrm{epi}_{\geq}(J_\infty) $ if and only if there exists a pair of matrices $X \succ 0$ and $Y \in \mathbb{R}^{m \times n}$ such that $K = YX^{-1}$ and $(\gamma, Y, X) \in \mathcal{F}_\infty$, where the set $\mathcal{F}_\infty = \{(\gamma,Y,X): 
X\succ 0, \mathrm{aff}(\gamma, Y, X) \preceq 0\}$ ($\mathrm{aff}(\cdot)$ represents an affine operator) is convex defined by suitable LMIs arising from the KYP lemma.  %
Since the $\mathcal{H}_\infty$ cost function $J_\infty$ is subdifferentially regular (see \Cref{lemma:H_inf_some_local_Lipschitz}), the convexity of $\mathcal{F}_\infty$ and the smoothing mapping $K = YX^{-1}$ further allow us the confirm that any Clarke stationary point of $J_\infty$ is globally optimal. We refer the interested reader to \cite[Theorem 1]{guo2022global} and \cite[Corollary 4.1]{zheng2024benign} for~details.        


 





==> geometry-stabilization.tex <==

\section{Topology and Geometry of Stabilizing Policies}
\label{section:stablizing-policies}




\mehran{i suggest remove this part till the ``Given an LTI system ..." the title of the section suggests what we will discuss?}

Designing efficient and reliable algorithms for solving the optimal closed-loop parameterized policy problem requires addressing
issues pertaining to stability, initial conditions, and the geometry of the domain and the cost. %
In this section, we first discuss the topological properties of stabilizing policies and then equip them with relevant geometries to obtain Riemannian manifold structures that can be utilized for developing efficient algorithms. 
While we focus on the discrete-time LTI systems as summarized in \Cref{parameterization}, similar results hold for the continuous case and we will refer the interested reader to relevant references for details.


\subsection{Topology of Static State-feedback Policies}

Given an LTI system \eqref{eq:state-evolution}, represented with $(A,B) \in \Amatrices \times \Bmatrices$, the set of static stabilizing state-feedback policies $\mathcal{S} \subseteq \mathbb{R}^{m \times n}$ \eqref{eq:static-stabilizing-policies} has rich topological properties. For example, provided $(A,B)$ is stabilizable, we have $\mathcal{S} \neq \emptyset$ and any element of $\mathcal{S}$ can be identified with pole placement \citep{aastrom2021feedback}.   
Using the Jury stability criterion~\citep{jury1964theory} (the discrete-time version of the Routh–Hurwitz stability criterion \citep{parks1962new}), %
we can express $\mathcal{S}$ as a finite system of polynomial inequalities written in terms of the elements of $K \in \mathbb{R}^{m \times n}$. However, this set~of~polynomial inequalities is complicated and may not offer good insights on topological properties of $\mathcal{S}$.    


\begin{fact} \label{fact:path-connected}
    The set of stabilizing static state-feedback policies $\mathcal{S}$ in \eqref{eq:static-stabilizing-policies} is path-connected.
\end{fact}
\noindent This fact follows from the Lyapunov stability LMI criterion and a standard Schur complement argument. The domain $\stableK$ coincides with the image of the \emph{continuous} mapping $(L,P) \mapsto K = L P^{-1}$ over the following convex, and thereby path-connected, set 
\begin{equation} \label{eq:convexPL}
        \left\{(P,L)\mid P \succ 0,  \begin{bmatrix}
         P & AP + BL \\
         PA^\transpose +L^\transpose B^\transpose & P
    \end{bmatrix} \succ 0 \right\}.
    \end{equation}


    

In addition, it is known that $\stableK$ is unbounded when $m \geq 2$, and the topological boundary $\partial \stableK = \{K \in \Kmatrices \;|\; \rho(A+BK) =1\}$ is a subset of $\Kmatrices$. Furthermore, as a result of the continuity of eigenvalues in the entries of the matrix, we can argue that $\stableK$ is an open set in $\Kmatrices$.

This property is vital for devising algorithmic iterates that have to reach a minimizer from any initial point in $\mathcal{S}$. It can furthermore be shown that $\mathcal{S}$ is contractible.







\subsection{Background on Riemannian Geometry}
Before diving into the geometry of stabilizing policies, we will first introduce basic concepts from Riemannian geometry. More specialized topics will be introduced in their respective sections in this paper. 

Let us consider a smooth manifold $\mathcal{M} \subset \mathbb{R}^N$. For example, the set of stabilizing policies $\stableK$, as an open subset of $\mathbb{R}^{m \times n}$, is a smooth manifold.
We call any smooth function $c:\mathbb{R} \to \mathcal{M}$ a smooth curve. A tangent vector at $x \in \mathcal{M}$ is any vector $\dot{c}(0) = \frac{d}{dt}{c}(t)|_{t=0}$, where $c(\cdot)$ is a smooth curve passing through $x$ at $t=0$. The set of all such tangent vectors at $x$ is a vector space called the tangent space at $x$ denoted by $T_x \mathcal{M}$. Its dimension $\dim(T_x \mathcal{M})$ coincides with the dimension of the manifold. For open sets, such as $\stableK$, its tangent spaces identifies with the vector space it lies within: $T_K \stableK \equiv \mathbb{R}^{m \times n}$; this is referred to as the usual identification of the tangent space. The tangent bundle is the disjoint union of tangent spaces $T \mathcal{M} := \{(x,v):x \in \mathcal{M}, v \in T_x\mathcal{M}\}$.



Let $F: \mathcal{M} \to \mathcal{N} \subset \mathbb{R}^M$ be a smooth function between two smooth manifolds. If we perturb $x \in \mathcal{M}$ along a direction $v \in T_x\mathcal{M}$, then the perturbation of the output from $F(\cdot)$ is another tangent vector in $T_{F(x)} \mathcal{N}$; the linear mapping $\diff F_x:T_x \mathcal{M} \to T_{F(x)} \mathcal{N}$ is called the differential of $F$ at $x$. Precisely, we define 
\begin{equation*}
    \diff F_x(v) := \frac{d}{dt} \big|_{t=0} (F \circ c)(t)
\end{equation*} 
where $c(\cdot)$ is any smooth curve passing $x$ at $t=0$ with velocity $v$. 

Considering the open set, and hence smooth manifold, of Schur stable matrices $\mathcal{A}$, we define the Lyapunov mapping $\lyap: \mathcal{A} \times \mathbb{R}^{n \times n} \to \mathbb{R}^{n \times n}$ that sends the pair $(A,Q)$ to the unique solution $P$ of 
\begin{equation}\label{eq:lyap-gen}
P = A P A^\transpose + Q.
\end{equation}
The following lemma characterizes the differential of the Lyapunov mapping which is instrumental in geometric analysis of policies for linear systems.

\begin{lemma}\label[lemma]{lem:dlyap}
The differential of $\lyap$ at $(A,Q) \in \mathcal{A} \times \mathbb{R}^{n\times n}$ along $(E,F) \in T_{(A,Q)} (\mathcal{A} \times \mathbb{R}^{n\times n}) \equiv \mathbb{R}^{n \times n} \times \mathbb{R}^{n\times n}$ is
\begin{gather*}
    \diff \lyap_{(A,Q)}[E,F] =
    \lyap \big(A, E \lyap(A,Q) A^\transpose + A \lyap(A,Q) E^\transpose + F \big).
\end{gather*}
 For any $A \in \mathcal{A}$ and $Q, \Sigma \in \Amatrices$ we further have the so-called \emph{\lyaptrace} property,
 \[\tr{\lyap(A^\transpose,Q) \Sigma} = \tr{\lyap(A, \Sigma) Q}.\]
\end{lemma}


A Riemannian metric $\langle \cdot,\cdot \rangle_x: T_x \mathcal{M} \times T_x \mathcal{M} \to \mathbb{R}$ on a smooth manifold $\mathcal{M}$ is an inner product that smoothly varies in $x$ with $x \in \mathcal{M}$. 
We call $(\mathcal{M},\langle \cdot,\cdot \rangle)$ a Riemannian manifold and often add a supper-script to clarify specific Riemannian metrics. 
A (locally-defined) retraction is a smooth mapping $\mathcal{R}: \mathcal{T} \subset T\mathcal{M} \to \mathcal{M}$ where $\mathcal{T}$ is an open subset of $(x,0_x) \in \mathcal{T}$ for each $x \in \mathcal{M}$, and the curve $c(t) := \mathcal{R}(x, t v)$ satisfies $c(0)=x$ and $\dot{c}(0)=v$. 
Every Riemannian metric induces a natural unique retraction called the ``exponential mapping'' that sends $v$ to $c(t)$ where $c$ is the unique curve with zero acceleration. However, one may adopt other retractions that may be cheaper to compute in the context as we will see in \S\ref{section:LQ-performance}.







\subsection{Geometry of Static State-feedback Policies}\label{subsec:geometry-static-policies}

 
The geometric information of a given optimization problem may be captured by designing a relevant Riemannian metric. Incorporating the geometric information may lead to faster convergence rates compared to ordinary optimization procedures.


Next, at any static feedback policies $K \in \stableK$, we define the following inner product that depends on a solution of a Lyapunov equation\footnote{Compare with the Frobenius inner product $\tensor{V}{W}{}^\texttt{F} = \tr{V^\transpose W}$ which induces the so-called Euclidean geometry.}:
\begin{equation*}
    \tensor{V}{W}{K}^{\texttt{L}} \coloneqq \tr{V^\transpose  W  Y_K},
\end{equation*} where $Y_K := \lyap(A+ BK , \Sigma)$. In fact, this dependence varies smoothly in policy $K$ and thus we can show that $\tensor{\cdot}{\cdot}{}^\texttt{L}$ is a Riemannian manifold referred to as the ``Lyapunov metric.'' \spencer{perhaps a sentence offering the intuition behind this. what is $Y_K$? why is $Y_K$ important? Why not, for instance, $P_K$?}



\begin{theorem}\label{thm:Riemannian-metric}
If $\Sigma \succ 0$ then $(\stableK,\tensor{\cdot}{\cdot}{}^\texttt{L})$ is a Riemannian manifold.\
\end{theorem}


\begin{figure}
    \centering
    \includegraphics[width = 0.45\textwidth]{figures/static_constrained_manifold.pdf}
    \caption{The (2-dimensional) set $\tilde{\stableK} = \stableK \cap \constraint$ of stabilizing policies subject to the diagonal sparsity constraint $\mathrm{D}=\{(1,1),(2,2)\}$. The LTI system is $A = \begin{pmatrix}0.8 &1\\0 & 0.8\end{pmatrix}$ and $B = \begin{pmatrix}0 &1\\1 & 0\end{pmatrix}$. 
    }
    \label{fig:SLQR-landscape}
\end{figure}


\subsection{Constrained Static State-feedback Policies} \label{subsec:constrained-policies}

In this section, we consider the policy family of static state-feedback policies under linear constraints. We can characterize this geometrically as follows. Let $\constraint \subset \mathbb{R}^{m \times n}$ be an affine subspace. Then our parameterization space will be $\Theta = \substableK \coloneqq \stableK \cap \constraint $. For instance, $\constraint$ could represent a prescribed sparsity pattern in \ac{slqr} problem or a static output-feedback in the \ac{olqr} problem \citep{talebi_riemannian_2022}. 


It is not always the case that a subset of a smooth manifold is itself an embedded submanifold. For example, this is not the case for the rationals as a subset of the reals. Fortunately, we can show that $\tilde{\mathcal{S}}$ is an embedded submanifold. This is done by showing that the inclusion map $\iota: \tilde{\mathcal{S}} \to \stableK$ is an immersion and a topological embedding i.e. it is injective, smooth, the  differential is everywhere injective, and $\iota$ is a homeomorphism onto its image.

From a \textit{topological} perspective, $\substableK \subset \stableK$ remains relatively open as $\stableK$ was open in $\Kmatrices$. However, in general, $\substableK$ is not only non-convex \citep{ackermann_parameter_1980} but also disconnected~\citep{feng_exponential_2019}. In fact, it may contain exponentially many disconnected components. As such, iterative procedures relying on connectivity of the domain may only provide local convergence guarantee.  
From a geometric perspective, this linear structure is only used to determine a computationally efficient ``local retraction'' which is achieved by proposing the so-called ``stability certificate'' that will be proposed in \S\ref{section:LQ-performance}. 

\subsubsection{SLQR}
Next, we discuss the submanifold induced in the \ac{slqr} problem. Any desired sparsity pattern on the policy $K$ imposes a linear constraint set, denoted by $\constraint_D$, which indicates a linear subspace of $\Kmatrices$ with nonzero entries only for a prescribed subset $D$ of entries. This means that for any $K \in \constraint_D$, we must have $[K]_{i,j}=0$ whenever $(i,j) \notin D$. 
\begin{fact}
    Any sparsity constraint $\constraint_D$ with $D \subset [m] \times [n]$ results in a properly embedded submanifold $\substableK = \stableK \cap \constraint_D \subset \stableK$ of dimension $|D|$. Also, each tangent space at $K \in \substableK$ can be canonically identified as $T_K\substableK \cong \constraint_D$.
\end{fact}
\noindent This fact follows by Submersion Level Set Theorem \cite{lee_introduction_2018}, where one can show that $\substableK$ in fact coincides with the zero level set of a smooth submersion (a smooth mapping whose differential is surjective everywhere); precisely, we define the mapping $\Phi\colon K \mapsto K^\circ \in \mathbb{R}^{mn-|D|}$ where $K^\circ$ is the vector of nonzero entries of $K$ in a fixed order, then $\substableK = (\Phi|_{\stableK})^{-1}(0)$. For a numerical example of this submanifold of $\stableK$, \Cref{fig:SLQR-landscape} illustrate a 2-by-2 example where policies $K$ are constrained to be diagonal.  See \cite{talebi_riemannian_2022} for the details.


\subsubsection{OLQR} Next, we discuss another constraint arising in \ac{olqr} problems with static output-feedback policies. The \ac{olqr} problem can be formulated similar to \cref{eq:LQR-policy-optimization} but with (noiseless) partial observations  $y_t= Cx_t$ where $C \in \Cmatrices$ is a prescribed output matrix (not the identity matrix). In this case, the feasible parameters takes the form of $\substableK = \stableK \cap \constraint_C$ where the constraint set $\constraint_C$ is defined as
\begin{gather*}
    \constraint_C \coloneqq \big\{K \in \Kmatrices \;|\; K = L C, \; L \in \Lmatrices \big\}.
\end{gather*}
\begin{fact}
    For any full rank output matrix $C$, the set of static output-feedback policies $\substableK = \stableK \cap \constraint_C$ is a properly embedded submanifold of $\stableK$ with dimension $md$. Also, each tangent space at $K \in \substableK$ identifies with $T_K\substableK \cong \constraint_C$.
\end{fact}
\noindent This fact also follows similarly by Submersion Level Set Theorem \cite{lee_introduction_2018}, but using another smooth submersion \(\Psi(K)\colon K \mapsto K(I_n - C^\dagger C),\) where $\dagger$ denotes the Moore-Penrose inverse. See \cite{talebi_riemannian_2022} for the details.









\subsection{Topology and Geometry of Dynamic Output-feedback Polices}

Herein, we focus on the output-feedback problem setup introduced in \S\ref{subsubsect:LQG}. Our parameterized family of policies will be the set of full-order dynamic output feedback policies $\Theta := \mathcal{C}_n$ in (\ref{eq:internallystabilizing}). We will discuss some topological and geometrical properties of this domain.

Similar to the static case, $\mathcal{C}_n$ is a nonconvex set. This is illustrated in \Cref{fig:feasible_region}.
It is also known that the set $\mathcal{C}_n$ is open and unbounded. Note that the same input-output behavior of a policy \eqref{eq:controller_discrete} can be represented using different state-space models, e.g., using different coordinates for the internal policy state. As mentioned in \Cref{subsection:geometry-manifold}, this is captured by the following notion of ``similarity transformations in control''. We let $\mathrm{GL}_n$ be the set of $n\times n$ invertible matrices. Define the mapping $\mathscr{T}_T\colon\mathrm{GL}_n\times\mathcal{C}_n\rightarrow\mathcal{C}_n$ that represents similarity transformations on $\mathcal{C}_n$ by
\begin{equation}\label{eq:def_sim_transform}
\mathscr{T}_T(\mK)
\coloneqq \begin{bmatrix}
I_m & 0 \\
0 & T
\end{bmatrix}\begin{bmatrix}
0 & C_{\mK} \\
B_{\mK} & A_{\mK}
\end{bmatrix}\begin{bmatrix}
I_p & 0 \\
0 & T
\end{bmatrix}^{-1} = \begin{bmatrix}
0 & C_{\mK}T^{-1} \\
TB_{\mK} & TA_{\mK}T^{-1}
\end{bmatrix}.
\end{equation}
Then, it is easy to verify that for any invertible matrix $T\in\mathrm{GL}_n$, the policy $\mK\in\mathcal{C}_n$ if and only if the transformed policy $\mathscr{T}_T(\mK) \in \mathcal{C}_n$. Indeed, the map
$
 \mK\mapsto \mathscr{T}_T(\mK)
$
is a diffeomorphism from $\mathcal{C}_n$ to itself for all such transformation $T\in\mathrm{GL}_n$.  
Besides the non-convexity, the set $\mathcal{C}_n$ can even be path disconnected, but it has at most two path-connected components. 

\begin{theorem} \label{Theo:disconnectivity}
The set ${\mathcal{C}}_{n}$ has at most two path-connected components.  
{If ${\mathcal{C}}_{n}$ has two path-connected components $\mathcal{C}_n^{(1)}$ and $\mathcal{C}_n^{(2)}$, then $\mathcal{C}_n^{(1)}$ and $\mathcal{C}_n^{(2)}$ are diffeomorphic under the mapping $\mathscr{T}_T$, for any invertible matrix $T\in\mathbb{R}^{n\times n}$ with $\det T<0$. 
}
\end{theorem}



The proof of this result is conceptually similar to the strategy in \eqref{eq:convexPL}, but with another classical (yet complicated) change of variables for dynamic policies (see, e.g.,~\citep{scherer1997multiobjective}). 
The potential disconnectivity comes from the fact that the set of real invertible matrices $\mathrm{GL}_n=\{\Pi\in\mathbb{R}^{n\times n}\mid\,\det \Pi\neq 0\}$ has two path-connected components:
$
\mathrm{GL}^+_n=\{\Pi\in\mathbb{R}^{n\times n}\mid\,\det \Pi> 0\},
\,
\mathrm{GL}^-_n=\{\Pi\in\mathbb{R}^{n\times n}\mid\,\det \Pi< 0\}.
$ In other words, the nature of similarity transformations may cause $\mathcal{C}_n$ to be disconnected.
The following results provide conditions that ensure $\mathcal{C}_n$ to be path-connected.  

\begin{theorem} %
If there exists a reduced-order stabilizing policy for \eqref{eq:dynamics_discrete}, \emph{i.e.}, ${\mathcal{C}}_{n-1} \neq \varnothing$, then $\mathcal{C}_n$ is path-connected. The converse also holds for systems with single-input or single-output, i.e., when $m=1$ or $p=1$ in \eqref{eq:dynamics_discrete}.
\end{theorem}


We can immediately deduce the following facts: 1) For any open-loop unstable first-order dynamical system, \emph{i.e.}, $n = 1$ and $A > 0$, there exist no reduced-order stabilizing policies, \emph{i.e.},   $\mathcal{C}_{n-1} = \varnothing$; thus its associated set of stabilizing policies $\mathcal{C}_n$ must be path disconnected. 2) For any open-loop stable systems, i.e., when $A$ is stable, we naturally have a reduced-order stabilizing policy, and thus the corresponding set of stabilizing policies is always path-connected. 
\Cref{fig:feasible_region} provides numerical examples for each case.



\begin{figure}[t]
\centering
    \includegraphics[width = 0.4\textwidth]{figures/dynamic_controller_manifold_disconnected_trans.pdf}
    \hspace{15mm}
    \includegraphics[width=0.4\textwidth]{figures/dynamic_controller_manifold_connected_trans.pdf}

    \caption{Illustration of the set of dynamic stabilizing policies $\mathcal{C}_1$ for an LTI system with $B = C = 1$ and: (a) with $A=1.1$ resulting in two path-connected components; (b) with $A=0.9$ resulting in one path-connected component. The reflectional symmetry with respect to the $B_K = C_K$ plane is due to the invariance under similarity transformations in \cref{eq:def_sim_transform}.}
    \label{fig:feasible_region}
\end{figure}






\subsection{Symmetries of Dynamic Output-feedback Policies: a Quotient Geometry}\label{subsubsec:invariants_of_feedback_policies}

\lina{this section is too long not easy for readers to get the flow. considering to add paragraph{} phrases.}\spencer{I agree... I shortened it. How do this look?}
Herein, we will describe an alternative parameterization for dynamic output-feedback systems (\ref{eq:internallystabilizing}) by turning $\mathcal{C}_n$ into a Riemannian manifold. 





The group of similarity transformations $\{\mathscr{T}_T(\cdot):T \in \mathrm{GL}_n\} \equiv \mathrm{GL}_n$ is a group action over $\mathcal{C}_n$. This induces an equivalence relation over $\mathcal{C}_n$: $\mK \sim \mK'$ if and only if there exists $T \in \mathrm{GL}_n$ such that $\mathscr{T}_T(\mK)=\mK'$. Note we are treating the open subset $\mathcal{C}_n \subset \mathbb{R}^{(n + m) \times (n + p)}$ as a smooth manifold.

The orbit of $\mK \in \mathcal{C}_n$ is the collection of controllers reachable from $\mK$ via similarity transformation:
\begin{equation*}
    [\mK]:=\left\{\begin{bmatrix} 0 & C_{\mK}T^{-1} \\ TB_{\mK} & TA_{\mK}T^{-1} \end{bmatrix}: T \in \mathrm{GL}_n \right\}.
\end{equation*} This is shown in Figure \ref{fig:controller_orbit_space}. Recall that LQG cost is constant on each orbit; this serves as the basis for the PO for LQG over the so-called quotient space in \S\ref{subsection:symmetry-manifold-structures-LQG}.


\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/dynamic_controller_manifold_with_orbits.pdf}
    \caption{The region of stabilizing dynamic feedback controllers $\mathcal{C}_1 \subset \mathbb{R}^3$ for the plant $(A,B,C)=(1.1,1,1)$. Each colored curve (red, purple, yellow, magenta, dark blue) is an individual orbit of policies. Note that $\mathcal{C}_1$ has 2 path-connected components.}
    \label{fig:controller_orbit_space}
\end{figure}



The quotient set (also known as the orbit set) of $\mathcal{C}_n$ is simply the collection of all orbits:
\begin{equation*}
    \mathcal{C}_n/\mathrm{GL}_n := \{[\mK] : \mK \in \mathcal{C}_n\}.
\end{equation*} We equip $\mathcal{C}_n/\mathrm{GL}_n$ with the induced quotient topology, defined as the finest topology in which the quotient map \begin{equation*}
    \pi:\mathcal{C}_n \to \mathcal{C}_n/\mathrm{GL}_n, \pi(\mK):=[\mK],
\end{equation*} is continuous. The resulting topological space is called the quotient or orbit space. 



The next step is to design a smooth structure for $\mathcal{C}_n/\mathrm{GL}_n$, turning it into a smooth manifold. For arbitrary quotient spaces, if there exists a smooth structure in which the quotient map is a smooth submersion, we call the resulting quotient space a smooth quotient manifold. In this context, the original smooth manifold is called the total manifold. %
Unfortunately, quotient spaces are often not even Hausdorff. Recall a  topological space is Hausdorff when any pair of points can be separated into disjoint neighborhoods of the corresponding points; this property implies all sequences have a unique limit. Therefore for non-Hausdorff quotient spaces, optimization is hopeless because limits cannot even be defined!

As it turns out, $\mathcal{C}_n/\mathrm{GL}_n$ is non-Hausdorff. The reason is the existence of non-controllable and non-observable, yet stabilizing, dynamic controllers which acts as `jumps''. This is explained in more detail in \cite{hazewinkel_moduli_1976}. Fortunately, the quotient space $\mathcal{C}_n^{\min}/\mathrm{GL}_n$ is Hausdorff \cite[Lemma 4.1]{kraisler2024output}.
Here, $\mathcal{C}_n^{\min}$ are all full-order policies with controllable and observable state space form. This follows from the remarkable theorem in \cite{hazewinkel_moduli_1976} proving the orbit space of minimal linear systems admits a smooth quotient manifold structure. It follows from this that $\dim(\mathcal{C}_n^{\min}/\mathrm{GL}_n)=nm+np$, an order of magnitude smaller. So, in the context of smooth optimization, we have a significantly smaller search space. 







Before we continue, let us discuss the tangent space of $\mathcal{C}_n$. Similar to the approach \S\ref{subsec:geometry-static-policies}, as an open subset, the tangent space of $\mathcal{C}_n$ coincides with its linear span: tangent \textit{vectors} to the open set $\mathcal{C}_n$ are simply 
\begin{equation*}
    \mathbf{V} = \begin{bmatrix} 0 & G \\ F & E\end{bmatrix}
\end{equation*} for any matrices $E \in \mathbb{R}^{n \times n}$, $F \in \mathbb{R}^{n \times p}$, and $G \in \mathbb{R}^{m \times n}$. Let us call this set $\mathcal{V}_q$. So, we can write $T_K \mathcal{C}_n \equiv \mathcal{V}_q$ for any $\mK \in \mathcal{C}_n$. 

In order to adopt smooth optimization techniques for $\mathcal{C}_n^{\min}/\mathrm{GL}_n$, we at last must equip the smooth quotient manifold with a retraction and Riemannian metric. To do this, we will discuss a correspondence between these two constructs between the total manifold $\mathcal{C}_n^{\min}$ and the quotient manifold $\mathcal{C}_n^{\min}/\mathrm{GL}_n$. It is easy to show that there is an invertible correspondence between Riemannian metrics on $\mathcal{C}_n^{\min}/\mathrm{GL}_n$ and \textit{similarity-invariant} Riemannian metrics on $\mathcal{C}_n^{\min}$. By this, we mean
\begin{equation}
    \langle \mathbf{V}, \mathbf{W} \rangle_{\mK} = \langle \mathscr{T}_T(\mathbf{V}), \mathscr{T}_T(\mathbf{W}) \rangle_{\mathscr{T}_T(\mK)} \label{eq:metric-inv}.
\end{equation} The same correspondence holds for \textit{similarity-equivariant} retractions
\begin{equation}
    \mathscr{T}_T(\mathcal{R}_\mK(\mathbf{V})) = \mathcal{R}_{\mathscr{T}_T(\mK)} (\mathscr{T}_T(\mathbf{V})). \label{eq:retraction-inv}
\end{equation} These two correspondences are as follows

\begin{subequations}\label{eq:quotient_structures}
    \begin{align}
        \langle \xi, \eta \rangle_{[\mK]}^{\text{quotient}} &:= \langle \lift_\mK(\xi), \lift_\mK(\eta) \rangle_{\mK}^{\text{total}} \\
        \mathcal{R}_{[\mK]}^{\text{quotient}}(\xi) &:= \mathcal{R}_\mK^{\text{total}}(\lift_\mK(\xi)).
    \end{align}
\end{subequations} Here, $\lift_\mK: T_{[\mK]} \mathcal{C}_n^{\min}/\mathrm{GL}_n \to \mathcal{V}_n$ is the lift operator defined in \cite[Def. 9.25]{boumal_introduction_2023}, and we used the keywords \textit{quotient} and \textit{total} to distinguish the two Riemannian structures. Therefore, such Riemannian constructs on the quotient manifold $\mathcal{C}_n^{\min}/\mathrm{GL}_n$ are completely characterized by such constructs defined on $\mathcal{C}_n^{\min}$ satisfying (\ref{eq:metric-inv}) and (\ref{eq:retraction-inv}). 



Since $\mathcal{C}_n^{\min} \subset \mathbb{R}^{(n + m) \times (n + p)}$ is an open set, a locally-defined retraction of choice is the Euclidean retraction: $\overline{\mathcal{R}}_{\mK}(\mathbf{V}) := \mK + \mathbf{V}$. Note that the Euclidean retraction is similarity-equivariant (\ref{eq:retraction-inv}). 







Now we will define a similarity-invariant Riemannian metric (\ref{eq:metric-inv}). Let $A_\cl(\mK),B_\cl(\mK), C_\cl(\mK)$ denote the closed-loop system matrices written in (\ref{eq:closed_loop_system}). A consequence of the minimality of any $\mK \in \mathcal{C}_n^{\min}$ is (1) $A_\cl(\mK)$ is Hurwitz and (2) the closed loop system $(A_\cl(\mK),B_\cl(\mK),C_\cl(\mK))$ is also minimal. The latter follows from the Popov-Belevitch-Hautus test. As a result, the controllability and observability Grammains of the closed-loop system satisfy 
\begin{subequations}
    \begin{align}\label{eq:pos_def_grammians}
        \mathcal{W}_c(\mK) &:= \lyap(A_\cl(\mK), B_\cl(\mK)B_\cl(\mK)^\transpose ) > 0\\
        \mathcal{W}_o(\mK) &:= \lyap(A_\cl(\mK), C_\cl(\mK)^\transpose C_\cl(\mK)) > 0.
    \end{align}
\end{subequations} 
Now, we introduced the so-called Krishnaprasad-Martin (KM) metric defined as
\begin{subequations}\label{eq:KM-metric}
\begin{align}
    \langle \mathbf{V}_1, \mathbf{V}_2 \rangle_\mK^{\texttt{KM}} &:= w_1 \text{tr}[\mathcal{W}_o(\mK) \cdot \mathbf{E}(\mathbf{V}_1) \cdot \mathcal{W}_c(K) \cdot \mathbf{E}(\mathbf{V}_2)^T] \\
    &+ w_2 \text{tr}[\mathbf{F}(\mathbf{V}_1)^T \cdot \mathcal{W}_o(\mK) \cdot \mathbf{F}(\mathbf{V}_2)] \\
    &+ w_3 \text{tr}[\mathbf{G}(\mathbf{V}_1) \cdot \mathcal{W}_c(\mK) \cdot \mathbf{F}(\mathbf{V}_2)^T] 
\end{align}
\end{subequations} where $w_1>0$ and $w_2,w_3 \geq 0$ are design constants and 
\begin{align*}
    \mathbf{E}(\mathbf{V}) := \begin{bmatrix} 0 & BG \\ FC & E \end{bmatrix}, \quad
    \mathbf{F}(\mathbf{V}) := \begin{bmatrix} 0 & 0 \\ 0 & F\end{bmatrix}, \quad 
    \mathbf{G}(\mathbf{V}) := \begin{bmatrix} 0 & 0 \\ 0 & G \end{bmatrix}.
\end{align*}
By referring to the properties in (\ref{eq:pos_def_grammians}) for each $K\in\mathcal{C}_n^{\min}$, we can establish the following result (analogous to the Riemannian metric in \Cref{thm:Riemannian-metric}).

\begin{theorem}\label{thm:Riem-metric-dynamic}\cite[Thm. 3.2]{kraisler2024output}
   The mapping that sends each $\mK \in \mathcal{C}_n^{\min}$ to the 2-tensor $\langle ., . \rangle^{\texttt{KM}}$ is a well-defined Riemannian metric over $\mathcal{C}_n^{\min}$, and the KM metric is similarity-invariant, i.e. satisfies (\ref{eq:metric-inv}).
\end{theorem}

Now that we have a similarity-invariant Riemannian metric (\ref{eq:metric-inv}), and a similarity-equivariant retraction (\ref{eq:retraction-inv}), we also can induce such structures onto $\mathcal{C}_n^{\min}/\mathrm{GL}_n$ through (\ref{eq:quotient_structures}).




==> introduction.tex <==
\section{Introduction}
\label{intro}
Optimization and control have had a rich symbiotic relationship since their inception. This is not surprising as the current dominate perspective on control design highlights: the design process for a dynamic system involves formalizing the notion of ``best'' with respect to selectable system parameters\footnote{Whatever the ``best'' qualifier implies.}--followed by devising algorithms that optimize the design objective with respect to these parameters. 
The interaction between these two disciplines has also highlighted an important facet of control design, namely, which design objectives--with respect to a given parameterization of control system (or more generally, parameters in the overall design architecture)-- subsequently facilitate algorithmic developments while preserving engineering judgement. For example, it is common to see a family of solution strategies for a given control design problem, including open vs. closed loop, approaches based on variational~\citep{Liberzon2011-en} or dynamic programming~\citep{Bertsekas2012-oq}, and constructs such as co-state, value, and of course, {\em policy}~\citep{Bertsekas2011-hi,Bertsekas2017-fi}. Each of these formalisms offer insights into control design, that although in principle can be formalized as an optimization problem, but reflect distinct intricacies in designing systems that evolve over time, interact with their environments, and have memory. For example, system theoretic properties such as stability, minimality, and robustness, significantly ``spice up" not only the control design problem formulation but also the adopted strategies for their solution~\citep{Zabczyk_undated-jw,Sontag2013-hk}. 
A powerful abstraction in this plethora of design techniques is that of \textit{policy}, mapping what the system has done (in terms of its state or output measurements) to what can influence its subsequent behavior. Not only does the existence of an ``optimal'' policy reduce the complexity of control implementation (as the control input is a trajectory) at the expense of realizing feedback, but as it turns out, it also addresses one of the key features of control design, namely robustness~\citep{Skogestad2005-wi,Doyle2013-vh}.\lina{this sentence is unclear to me.}\mehran{just saying that feedback can address robustness to plant variations or more generally uncertainty in the design.} This survey aims to capture the {\em geometry} of policy optimization for a few iconic design techniques in control (including stabilization, linear quadratic control, and $\mathcal{H}_\infty$ robust control), capturing distinct facets of adopting such a perspective for feedback design. However, as we undertake such an endeavor, it is important to comment on the timeliness of this approach, as well as how it connects--and is distinct--from previous works, particularly in relation to its reference to ``geometry''.

Historically, the ``geometric'' qualifier has been used in systems and control to shed light on more subtle aspects of system design. In linear geometric control for example, subspace geometry is used to delineate upon coordinate-independence of system theoretic constructs such as controllability and observability\lina{there might be typos in the sentence. The sentence is unclear to me}\mehran{for example, the ideas is to talk about controllability without using the linear algebra involving $A$ and $B$, but using subspaces generated by the state and input maps; e.g., observability pertains to the dimension of the kernel of a composition map, etc. so it is essentially coordinate-free}~\citep{wonham_w_murray_linear_1985,Trentelman2001-ck}. Geometric nonlinear control, on the other hand,  characterizes notions such as controllability for nonlinear systems, by viewing their evolution in terms of vector fields, and then brings forth a differential geometric formalism for their analysis, e.g., differentiable manifold, distributions, and Lie algebras~\citep{Isidori2013-dj,Nijmeijer1990-xr}; the aim is to free control theory (analysis and synthesis) from the confinements of linearity and linear algebra via a coordinate-free analysis of dynamical systems. Using this geometric vista, linear maps are uplifted to diffeomorphisms, while notions
such as controllability matrix are revealed as Lie brackets~\citep{Brockett2014-zg}. As these two examples demonstrate, ``geometry'' is often used to hint at coordinate-independence of concepts, similar to how finite dimensional vector spaces are related to linear algebra. Other notable works in adopting a geometric perspective in systems and control theory, particularly in relation to realization theory and system identification include~\citep{beckmann_invariants_1976,byrnes_fine_1980,tannenbaum_invariance_1981}.

By including “geometry” in the title of this survey, we deliberately mean
to promote adopting a similar geometric perspective as the aforementioned works, but for the space of feedback control policies rather than system models or their trajectories, which highlights the importance of how one characterizes notions such as distance and direction for these policies.
Such a perspective not only complements other features of this space (in addition to its topological, analytic, or algebraic structures) but more importantly, has direct consequences for devising algorithms for the corresponding optimization problems.
This geometric perspective and its algorithmic implications have also been adopted in neighboring decision sciences, e.g., statistical learning and Markov Decision Processes (MDPs). Notable in the landscape of such geometric techniques, we mention the notion of natural gradients, where the geometry of the underlying model, singled out in the design objective, is systematically used to synthesize algorithms that behave invariant under certain re-parameterizations. By invariance, we mean embedding the underlying model with a notion of distance that is preserved under certain mappings, e.g., Fisher metric in statistical learning~\citep{amari_natural_1998,Amari2016-do}. Closely related to the present survey is adopting the theory of natural gradients for MDPs as first proposed in~\citep{Kakade2002-fc}, where the Hessian geometry induced by the entropy plays a central role in the
design and convergence analysis of the corresponding algorithms; also see~\citep{Agarwal2021-ss}. These geometric insights have a number of algorithmic and system-theoretic consequences. For example, as we will see, improving the policy by taking steps in the direction of its (negative) gradient proves to be an effective means of obtaining optimal policies, i.e., first-order policy updates. The ``zeroth" order version of the above scheme, on the other hand, leads to using function evaluations to approximate the corresponding gradients from data- say, when such evaluations can be obtained from an oracle that can return approximate values of the cost. Such a setup that closely relates to data-driven reinforcement learning.
Key questions in this data-driven realization of geometric first-order methods are how many function evaluations (and with what accuracy) and over how many iterations, an accurate estimate of the optimal policy can be obtained~\cite{Fazel2018-pv,Malik2019-bs,Mohammadi2021-vs,Mohammadi2020-iv}.\lina{I think we should break the paragraph to two and also streamline the flow. My mind started drifting when reading this paragraph. Need to have a more clear flow. Concise discussion should also be better to get message delivered.}

As such, the geometric perspective for policy optimization promoted in this survey, has other motivations in addition to being simply elegant. In particular, we believe that this point of view can serve the following purposes: (1) provide a more direct bridge between control synthesis and data-driven design paradigms such as reinforcement learning~\citep{Lewis2012-zf}, (2) it clarifies fundamental issues pertaining to how control design objectives interact with the feasible set of control parameters, e.g., stabilizing feedback policies, (3) why parameterizing control design should go hand in hand with the adopting the ``right" geometry, not only for developing algorithms, but shed light on issues such as conditioning and lower bounds. Lastly, we believe that this geometric perspective would allow foreseeing design and algorithmic challenges beyond classic paradigms involving quadratic costs and linear dynamics.\lina{this paragraph has some repetitive message compared to the previous paragaraph.}

The survey is structured as follows. In \S\ref{parameterization} we make the parameterization theme on control design alluded to above more explicit. While this perspective provides a direct approach to formalize policy optimization for control, it also underscores how the constraints imposed by system theoretic notions such as stabilizability make the feasible set of the optimization non-trivial. This is first more pursued for state-feedback, followed by that of dynamic feedback in \S\ref{section:stablizing-policies}. We then turn our attention to how distinct design performance measures interact with the feasible set of feedback policies in \S\ref{section:LQ-performance}.
Algorithmic implications and data-driven realizations of the geometric perspective on policy optimization are then examined under \S\ref{data-driven}. In \S\ref{summary}, we provide a summary of the key points put forth by this survey as well as our outlook on the future work; \S\ref{notes-commentary} provides commentary on references with contributions reflected in this survey.

\mehran{are we covering a lot?}


==> policy-optimization-ignore.tex <==
\section{Policy Optimization in Control--Role of Parameterization} \label{parameterization}

Control theory offers a principled use of feedback algorithms to influence and steer the behavior of a dynamical system in order to achieve a desired goal, while minimizing a certain performance cost. Let us consider a discrete-time dynamical system:
\begin{subequations}\label{rev-eq:system-dynamics}
    \begin{align}
        x_{t+1} &= f(x_t,u_t,w_t) \\
        y_t &= h(x_t,w_t)
    \end{align}
\end{subequations} Here, $x_t \in \mathbb{R}^n$ is the system state, $u_t \in \mathbb{R}^m$ is the control input, and $y_t \in \mathbb{R}^p$ is the system measurement. Next, $w_t$ is an external involuntary input to characterize non-linearities, system uncertainties, stochastic noise, or worse-case disturbance scenarios. 

At each time step $t$, we use $l(x_t,u_t)$ to denote the stage cost of the current state and input. We often assume $l$ is continuously differentiable and strictly convex. The goal of infinite-horizon optimal control is to choose $\mathbf{u}=(u_0,u_1,\ldots,)$ to minimize the average infinite-horizon cost:
\begin{equation}\label{rev-eq:ave-inf-hor-cost}
    J(\mathbf{u}; \mathbf{w}, x_0) = \lim_{T \to \infty} \frac{1}{T} \sum_{t=0}^T l(x_t,u_t),        
\end{equation} where $x_{t+1} = f(x_t,u_t,w_t)$ for $t \geq 0$ and $\mathbf{w}=(w_0,w_1,\ldots,)$. It should be noted the state trajectory $\mathbf{x}:=(x_0,x_1,\ldots)$ is built into the definition of $J$, which solely depends on the control input $\mathbf{u}$, the external disturbance $\mathbf{w}$, and initial state $x_0$. Often, $\mathbf{w}$ and $x_0$ will be treated as constants in some sense, and the only varying parameter will be $\mathbf{u}$. For example:
\begin{subequations}\label{rev-eq:single-param-ave-inf-hor-cost}
    \begin{align}
        J(\mathbf{u}) &:= \mathbb{E}_{\mathbf{w},x_0} J(\mathbf{u};\mathbf{w}, x_0)\\ 
        J(\mathbf{u}) &:=\sup_{\|\mathbf{w}\|_{l_2} \leq 1} J(\mathbf{u};\mathbf{w}, 0)
    \end{align}
\end{subequations}

\subsection{(Revision) Policy parameterization for closed-loop optimal control}

Instead of optimizing over a deterministic control sequence $\mathbf{u}$, which we call the \textit{optimal open-loop policy problem}, we optimize over a class of \textit{feedback policies} that depend on the system history: $\mathcal{H}_t := (u_{0:t-1}, y_{0:t}) \in \mathbb{R}^{m \times t} \times \mathbb{R}^{p \times (t + 1)}$, where $u_{0:t-1} := (u_0,u_1,\ldots,u_{t-1})$ and similar for $y_{0:t}$. The \textit{feedback} or \textit{closed-loop policy} at time $t$ $\pi_t:\mathbb{R}^{m \times t} \times \mathbb{R}^{p \times (t + 1)} \to \mathbb{R}^m$ will be a measurable function that maps the system history $\mathcal{H}_t$ at time $t$ to a deterministic control action $u_t$. We can alternatively define $\pi_t(\mathcal{H}_t)$ to be a distribution and set $u_t \sim \pi_t(\mathcal{H}_t)$. In this case, we would have to slightly augment (\ref{rev-eq:single-param-ave-inf-hor-cost}). We will call $\pi=(\pi_0,\pi_1,\ldots)$ the feedback policy. Let $\Pi$ be the infinite-dimensional vector space of all such feedback policies $\pi(\cdot)$. For notational brevity, we will often write $\pi(\mathcal{H}_t):=\pi_t(\mathcal{H}_t)$. Therefore, the \textit{optimal closed-loop policy problem} reads as 
\begin{subequations}\label{rev-eq:closed-loop-policy-prob}
    \begin{align}
        \min_{\pi \in \Pi} & \ J(\mathbf{u}) \\
        \text{s.t. } &(\ref{rev-eq:system-dynamics}) \\
        u_t &= \pi(\mathcal{H}_t) \\
        \mathcal{H}_t &= (u_{0:t-1},y_{0:t}),
    \end{align}
\end{subequations} where $J(\mathbf{u})$ is supposed to take any of the forms in (\ref{rev-eq:single-param-ave-inf-hor-cost}). Here, the decision variables are the polices $\pi(\cdot) \in \Pi$. 


Since it is non-trivial to optimize directly over this space $\Pi$, the so-called ``policy parameterization'' approach is to parameterize a subset of $\Pi$ with a finite set of parameters $\theta \in \Theta \subset \mathbb{R}^{n_p}$. That way, our parameterized family of policies $\{\pi_\theta(\cdot)\}_{\theta \in \Theta} \subset \Pi$ is finite-dimensional. Note that the forms of policy parameterization can be very flexible, such as linear dynamical systems, polynomials, kernels, or neural networks. As we will show below, it is known that a static linear map is sufficient for many optimal and robust control problems of linear time-invariant (LTI) systems \citep{zhou1996robust}. Then, the \textit{optimal closed-loop policy problem} \eqref{rev-eq:closed-loop-policy-prob} is simplified to one that aims to find the best \textit{parameterized} policy $\pi_\theta$:

\begin{equation} \label{rev-eq:closed-loop-param-policy-prob}
    \min_{\theta \in \Theta}  J(\theta). 
\end{equation} Here, we are treating 
\begin{equation}\label{param-policy}
    J(\theta)  := J(\mathbf{u}(\theta)),
\end{equation} where $u_t(\theta) := \pi_\theta(\mathcal{H}_t)$. We call (\ref{rev-eq:closed-loop-param-policy-prob}) the \textit{optimal closed-loop parameterized policy problem}. If $\pi^*$ solves (\ref{rev-eq:closed-loop-policy-prob}) and $\theta^*$ solves (\ref{rev-eq:closed-loop-param-policy-prob}), then it should be remarked $J(\pi^*) \leq J(\pi_{\theta^*})$. It should be noted we can explicitly incorporate a policy constraint on $\Theta$ that represents closed-loop stability $J(\theta) < \infty$ or certain information constraints. 

Conceptually, it appears simple and flexible to use local search algorithms, such as policy gradient or its variants, to seek the ``best'' policy for \eqref{rev-eq:closed-loop-param-policy-prob}. Once the corresponding cost in \eqref{rev-eq:closed-loop-param-policy-prob} can be estimated from sampled trajectories, this policy optimization setup indeed is very amenable for data-driven design paradigms such as reinforcement learning \citep{recht2019tour}. 
One goal of this article is to highlight some \textit{rich}, yet \textit{complicated} and \textit{intriguing}, geometry in policy optimization \eqref{rev-eq:closed-loop-param-policy-prob}, including nonconvexity, potentially disconnected feasible domain $\Theta$, spurious stationary points of the cost $J$, symmetry, and smooth (Riemannian) manifold structures. Our focus will be on classic and iconic control tasks for linear time-invariant (LTI) systems, including stabilization, LQR, LQG, and  $\mathcal{H}_\infty$ robust control. These geometrical understandings will often provide insights for designing principled local search algorithms to solve \eqref{rev-eq:closed-loop-param-policy-prob}, such as policy gradient methods with global/local convergence guarantees \citep{fazel2018global,mohammadi2021convergence,hu2023toward}. Inspired by the rich geometry in \eqref{rev-eq:closed-loop-param-policy-prob}, we will further emphasize that a ``complete policy parameterization'' should come with an associated metric, capturing the inherent geometry, which may help improve the problem's conditioning \citep{kraisler2024output,talebi_riemannian_2022}.   




\subsubsection{(Revision) Linear Quadratic Regulator (LQR)}


For the LQR problem, the system dynamics \eqref{rev-eq:system-dynamics} read as 
\begin{equation} \label{eq:state-evolution}
    {x}_{t+1}= Ax_t+Bu_t+ w_t, \qquad y_t = C x_t.
\end{equation} where $C=I$ is the identity matrix, $x_t \in \mathbb{R}^n, u_t \in \mathbb{R}^m$ are the system state and input, and $w_t$ is a discrete-time white-noise process with a stationary full-rank covariance matrix $\Sigma \succ 0$. In \eqref{eq:state-evolution}, we assume that the state is directly observed. This implies the system history takes the form $\mathcal{H}_t = (u_{0:t-1}, x_{0:t})$. Given performance weights $Q \succeq 0, R \succ 0$, the fixed initial point stochastic \textit{optimal closed-loop policy problem} (\ref{rev-eq:closed-loop-policy-prob}) is
\begin{subequations}\label{rev-eq:LQR-noise}
    \begin{align}
    &\min_{\pi \in \Pi} \mathbb{E}_{\mathbf{w}} J_{2}(\mathbf{u}; \mathbf{w}, 0) \\
    &\text{s.t. } (\ref{eq:state-evolution}), u_t = \pi(\mathcal{H}_t) \\
    &\mathcal{H}_t = (u_{0:t}, x_{0:t-1})
    \end{align} 
\end{subequations} where $J_{2}$ is the infinite-horizon cost (\ref{rev-eq:ave-inf-hor-cost}) with $l(x_t,u_t)=\frac{1}{2}(x_t^TQx_t + u_t^TRu_t)$.

Note that the cost in \Cref{rev-eq:LQR-noise} is oblivious to any bounded initial condition $x_0$ as long as the policy is stabilizing. 

Alternatively, when the dynamics is noiseless but the initial condition is uncertain, we might be interested in minimizing the following objective instead 
\begin{subequations}\label{rev-eq:LQR-noiseless}
    \begin{align}
        &\min_{\pi \in \Pi} \mathbb{E}_{x_0} J_2(\mathbf{u}; \mathbf{0}, x_0) \\
        &\text{s.t. } (\ref{eq:state-evolution}), u_t = \pi(\mathcal{H}_t) \\
        &\mathcal{H}_t = (u_{0:t}, x_{0:t-1})
    \end{align}
\end{subequations} where $x_0$ is drawn from a distribution with covariance $\Sigma \succ 0$. We will see later that both of the problems in \Cref{rev-eq:LQR-noise} and \Cref{rev-eq:LQR-noiseless} essentially amount to the same policy optimization problem.

A remarkable property of the closed-loop optimal policy problem is the optimal policy $\pi^*$, when it exists, is linear in the state and depends only on the current state. That is, $\pi^*(\mathcal{H}_t) = \pi^*(x_t) = K x_t$ for some $K \in \mathbb{R}^{m \times n}$. 

Inspired by this property, for both  \eqref{rev-eq:LQR-noise} and \eqref{rev-eq:LQR-noiseless}, we can parameterize the LQR policy as a linear mapping as $u_t = Kx_t, K \in \mathbb{R}^{m \times n}$. Then, the set of stabilizing static state-feedback policies is  
\begin{equation} \label{eq:static-stabilizing-policies}
    \Theta := \mathcal{S} = \{K \in \mathbb{R}^{m \times n}: \rho(A+BK) < 1\}.
\end{equation} where $\rho(\cdot)$ denotes the spectral radius of a square matrix. Following (\ref{param-policy}), we can define $J_2$ over $\mathcal{S}$, where $J_2(K)$ is corresponding to the objective in either~\eqref{rev-eq:LQR-noise} or \eqref{rev-eq:LQR-noiseless}. Our parameterized policy family will be $\{\pi_K\}_{K \in \mathcal{S}}$ with $\pi_K(\mathcal{H}_t) := K x_t$. Last, the \textit{optimal closed-loop parameterized policy problem} \eqref{rev-eq:closed-loop-param-policy-prob} for LQR becomes 
\begin{equation}
\begin{aligned} \label{eq:LQR-policy-optimization}
    \min_{K} \quad & J_{2}(K) \\
    \mathrm{subject~to}\quad &  K \in \mathcal{S}. 
\end{aligned} 
\end{equation}

\subsubsection{(Revision) Linear Quadratic Gaussian (LQG) Control}

We here specify the general closed-loop optimal policy problem \eqref{rev-eq:closed-loop-policy-prob} in the context of LTI systems with partial observation:
\begin{equation} \label{eq:dynamics_discrete}
    \begin{aligned}
        x_{t+1} &= A x_t + B u_t + w_t, \\
        y_t &= Cx_t + v_t, 
    \end{aligned}
\end{equation}
where $x_t \in \mathbb{R}^n, u_t \in \mathbb{R}^m, y_t \in \mathbb{R}^p$ are the system state, input, and output measurement at time $t$, and $w_t \sim \mathcal{N}(0, W), v_t \sim \mathcal{N}(0, V)$ are Gaussian process and measurement noises, respectively.  It is assumed that the covariance matrices satisfy $W \succeq 0, V \succ 0$.
Given performance weight matrices $Q \succeq 0, R \succ 0$, the closed-loop optimal policy problem (\ref{rev-eq:closed-loop-policy-prob}) is
\begin{subequations}\label{LQG-policy-problem}
    \begin{align}
        &\min_{\pi \in \Pi} \mathbb{E}_{\mathbf{w}} J_2(\mathbf{u};\mathbf{w},0) \\
        &\text{s.t. } (\ref{eq:dynamics_discrete}), u_t = \pi(\mathcal{H}_t) \\
        & \mathcal{H}_t = (u_{0:t-1}, y_{0:t})
    \end{align}
\end{subequations} It should be noted that the only difference between the optimal closed-loop policy problems (\ref{LQG-policy-problem}) and (\ref{rev-eq:LQR-noise}) is the policies are constrained to depend on output-feedback $(u_{0:t-1},y_{0:t})$ and state-feedback $(u_{0:t-1},x_{0:t-1})$, respectively. 


Next, we will construct a parameterized family of policies with LTI systems in state-space form:
\begin{equation} \label{eq:controller_discrete}
    \begin{aligned}
        \xi_{t+1} &= A_{\mK} \xi_t + B_{\mK} y_t, \\
        u_t &= C_{\mK} \xi_{t},
    \end{aligned}
\end{equation}
where $\xi_t \in \mathbb{R}^q$ is the policy internal state at time $t$, and policy parameters $(A_{\mK},B_{\mK},C_{\mK}) \in \mathbb{R}^{q \times q} \times \mathbb{R}^{q \times p} \times \mathbb{R}^{m \times q}$ specify the policy dynamics. If $q = n$, we refer to \eqref{eq:controller_discrete} as a \textit{full-order} dynamic policy; if $q < n$, it is called a \textit{reduced-order} dynamic policy. In this survey, we will mostly focus on the case $q = n$ since it is known that full-order dynamic policies contain the globally optimal solution to the closed-loop optimal policy problem \eqref{LQG-policy-problem} \citep{zhou1996robust}. It follows our policy family is $\{\pi_{\mK}\}_{\mK \in \mathcal{C}_n}$ with $\pi_{\mK}(\mathcal{H}_t) := \sum_{i=1}^t C_{\mK} A_{\mK}^{i - 1}B_{\mK} y_{t - i }$, where we assume $\xi_0 = 0$.


Combining~\eqref{eq:controller_discrete} with~\eqref{eq:dynamics_discrete} leads to the closed-loop system below 
\begin{equation}\label{eq:closed_loop_system}
\begin{aligned}
   \begin{bmatrix} x_{t+1} \\ \xi_{t+1} \end{bmatrix} &= \begin{bmatrix}
    A & BC_{\mK} \\
    B_{\mK}C & A_{\mK}
    \end{bmatrix} \begin{bmatrix} x_t \\ \xi_t \end{bmatrix}  +  \begin{bmatrix} I & 0 \\ 0 & B_{\mK}  \end{bmatrix}\begin{bmatrix} w_t \\ v_t \end{bmatrix} \\
    \begin{bmatrix} y_t \\ u_t \end{bmatrix}& = \begin{bmatrix} C & 0 \\ 0& C_{\mK} \end{bmatrix} \begin{bmatrix} x_t \\ \xi_t \end{bmatrix} + \begin{bmatrix} v_t \\0 \end{bmatrix}.
\end{aligned}
\end{equation}
The set of stabilizing controllers with order $q \in \mathbb{N}$ is defined as %
\begin{equation} \label{eq:internallystabilizing}
    \Theta := \mathcal{C}_{q} = \left\{
    \left.\mK=\begin{bmatrix}
    0_{m\times p} & C_{\mK} \\
    B_{\mK} & A_{\mK}
    \end{bmatrix}
    \in \mathbb{R}^{(m+q) \times (p+q)} \right|\;  \rho\left(\begin{bmatrix}
    A & BC_{\mK} \\
    B_{\mK}C & A_{\mK}
    \end{bmatrix}\right) < 1\right\},
\end{equation}

Like in the LQR setup, we similarly follow (\ref{param-policy}) and define $J_2(\mK):=\mathbb{E}_{\mathbf{w}, x_0} J(\mathbf{u}; \mathbf{w}, x_0)$, where $u_t:= \pi_{\mK}(\mathcal{H}_t)$. Given the dimension $n$ of the state variable of the plant, the optimal closed-loop parameterized policy problem (\ref{rev-eq:closed-loop-param-policy-prob}) is
\begin{equation} \label{eq:LQG_policy-optimization}
    \begin{aligned}
        \min_{\mK \in \mathcal{C}_n} \quad &J_2(\mK) \\
    \end{aligned}
\end{equation}



Throughout this survey, we make the standard assumption that $(A,B)$ is stabilizable and $(C,A)$ is detectable for the LTI system \eqref{eq:dynamics_discrete}, so that $\mathcal{C}_n$ is nonempty.  



\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width = 0.24\textwidth]{figures/3d_policy_11.png}}
    \subfigure[]{\includegraphics[width = 0.24\textwidth]{figures/3d_policy_21.png}}
    \subfigure[]{\includegraphics[width = 0.24\textwidth]{figures/3d_policy_12.png}}
    \subfigure[]{\includegraphics[width = 0.24\textwidth]{figures/3d_policy_22.png}}
    \caption{The nonconvex (4-D) set of stabilizing policies $\stableK$ in \eqref{eq:static-stabilizing-policies} with $A = \begin{bmatrix}1 &1\\0 & 1\end{bmatrix}$ and $B = \begin{bmatrix}0 &1\\1 & 0\end{bmatrix}$. We illustrate the intersection of $\stableK$ with the affine subspaces that are passing through $K_0 = -\begin{bmatrix}0 &0.8\\0.9 & 0.9\end{bmatrix}$ and are orthogonal to the direction $E$ where  
    (a) $E = \begin{bmatrix}1 &0\\0 & 0\end{bmatrix}$, (b) $E = \begin{bmatrix}0 &1\\0 & 0\end{bmatrix}$, 
    (c) $E = \begin{bmatrix}0 &0\\1 & 0\end{bmatrix}$, and (d) $E = \begin{bmatrix}0 &0\\0 & 1\end{bmatrix}$. \shahriar{improve the labels... the color is horrible.}}
    \label{fig:LQR-simple}
\end{figure}


\subsubsection{(Revision) $\mathcal{H}_\infty$ robust control}

When the disturbance $w_t$ in system \eqref{eq:state-evolution} is not stochastic but adversarial with bounded energy, e.g., $\|w\|_{L_2}^2 \coloneqq \sum_{t=0}^\infty w_t^\transpose w_t \leq 1$, one typical control goal is to design a sequence of control inputs $u_t$ that improve the worst-case performance (i.e., the closed-loop robustness). In classical control, the worst-case performance is typically measured by an $\mathcal{H}_\infty$ norm of a certain closed-loop channel, and thus this problem is known as $\mathcal{H}_\infty$ robust control.

The worst-case performance when $w_t$ has bounded energy less than or equal to 1 is measured~by 
\begin{equation} \label{eq:Hinf-cost-def}
    J_\infty(\mathbf{u}) := \sup_{\|\mathbf{w}\|_{l_2} \leq 1} J_2(\mathbf{u}; \mathbf{w}, 0),
\end{equation} where $Q \succeq 0, R \succ 0$ are given weights. Then, following (\ref{rev-eq:closed-loop-param-policy-prob}), we can equivalently express $J_\infty$ instead as a function on $\mathcal{S}$. 

The resulting optimal closed-loop policy problem (\ref{rev-eq:closed-loop-policy-prob}) is formulated as
\begin{equation*} %
    \begin{aligned}
        \min_{\pi \in \Pi} \quad & \sup_{\|\mathbf{w}\|_{l_2} \leq 1} J_2(\mathbf{u}; \mathbf{w}, 0) \\
        \text{subject to} \quad & ~\eqref{eq:state-evolution} \\
        u_t &= \pi(\mathcal{H}_t) \\
        \mathcal{H}_t &= (u_{0:t-1}, x_{0:t})
    \end{aligned}
\end{equation*}


We can again construct a parameterized family of polices by using static feedback matrices. So, $\Theta := \mathcal{S}$ and $\pi_K(\mathcal{H}_t) := Kx_t$. Then, we can set $J_\infty(K):= \sup_{\|\mathbf{w}\|_{l_2} \leq 1} J_2(\mathbf{u}(K); \mathbf{w}, 0)$, where $u_t(K) = \pi_K(\mathcal{H}_t)=Kx_t$. The resulting optimal closed-loop parameterized policy problem will then be
\begin{subequations}\label{eq:Hinf-policy-optimization}
    \begin{align}
        \min_{K \in \mathcal{S}} J_\infty(K)
    \end{align}
\end{subequations}

This problem \eqref{eq:Hinf-policy-optimization} is a state-feedback $\mathcal{H}_\infty$ control, where we can use a linear static policy with no loss of generality \citep{zhou1988algebraic}. As the partially observed LTI system \eqref{eq:dynamics_discrete} where the state $x_t$ is not directly measured, we can consider the general output-feedback $\mathcal{H}_\infty$ control, in which a dynamic policy similar to \eqref{eq:controller_discrete} is needed \citep{zhou1996robust}. At the time of writing, geometrical properties for output-feedback $\mathcal{H}_\infty$ control are under active investigation; see e.g., \citep{zheng2023benign,tang2023global,guo2024complexity}. We will not pursue the details here.     



==> policy-optimization-old.tex <==

\section{Policy Optimization in Control --- The Role of Parameterization} \label{parameterization}

Control theory offers a principled use of feedback algorithms to influence and steer the behavior of a dynamical system in order to achieve a desired goal, while minimizing a certain performance cost. Starting from an initial state $x_0$, let us consider a discrete-time dynamical system 
\begin{equation} \label{eq:general-dynamics}
\begin{aligned}
x_{t+1} &= f_t(x_t, u_t, w_t),  \\ 
y_t &= h_t(x_t, w_t), 
\end{aligned}
\end{equation}
where $x_t$ is the state of the system, $y_t$ is the output measurement of the system, $w_t$ is a random disturbance at time $t$, and $u_t$ is the control action (to be designed as a function of available input and measurement information up to time $t$); $f_t$ is a function representing the system dynamic update, and $h_t$ is the measurement function. At each time step $t$, we use $c(x_t, u_t)$ to denote the stage cost of the current $x_t$ and $u_t$. The goal of a infinite-horizon optimal control problem is to choose a sequence of control inputs $u_0, u_1, u_2, \ldots$ to minimize the following average cost performance 
\begin{equation} \label{eq:performance-measure}
J(\x,\u) = \lim_{T \to \infty}\, \mathbb{E}_{w_t} \left(\frac{1}{T}\sum_{t=0}^T c(x_t, u_t)\right),
\end{equation}
where we denote the state trajectory $(x_0, x_1, x_2, \ldots)$ and input sequence $(u_0, u_1, u_2, \ldots)$ as $\x$ and $\u$, respectively, for notational simplicity. Note that in general, the control inputs $u_0, u_1, u_2, \ldots$ should at least stabilize \eqref{eq:general-dynamics}; otherwise, the cost in \eqref{eq:performance-measure} would be infinite.


Mathematically, we aim to solve the following optimization problem 
\begin{equation}
\begin{aligned} \label{eq:general-optimal-control-new}
    \min_{\u} \quad & J(\x, \u) \\
    \mathrm{subject~to}\quad & \eqref{eq:general-dynamics}.
\end{aligned} 
\end{equation}
In the optimal control problem \eqref{eq:general-optimal-control-new}, for causality,  the control input $u_t$ at time $t$ is only allowed to use the history information $\mathcal{H}_t:= (u_0, \ldots, u_{t-1}, y_0, \ldots, y_{t})$. 

\subsection{Policy parameterization for optimal control} 
Typically, instead of optimizing over deterministic control sequences $u_t$, we optimize over \textit{policies} via feedback based on the history information $\mathcal{H}_t$ \citep{Bertsekas2012-oq,zhou1996robust}. A control policy is a \textit{function} $\pi$ that maps the history information $\mathcal{H}_t$ to a new control action $u_t$. Thus, a standard policy optimization for the optimal control \eqref{eq:general-optimal-control-new} reads as 
\begin{equation}
\begin{aligned} \label{eq:policy-control-new}
    \min_{\pi} \quad & J(\x, \u) \\
    \mathrm{subject~to}\quad & \eqref{eq:general-dynamics}, u_t = \pi(\mathcal{H}_t)
\end{aligned} 
\end{equation}
where the decision variables are the policies (i.e., functions) $\pi$. 

Since it is non-trivial to optimize directly over the space of functions (which is typically infinite-dimensional), 
the so-called ``policy parameterization'' approach is to parameterize the admissible class of feedback policies by a set of finite-dimensional parameters $\theta \in \mathbb{R}^{n_c}$ with $n_c \in \mathbb{N}$ as 
\begin{equation} \label{eq:policy-parameterization}
u_t = \pi_\theta(\mathcal{H}_t).
\end{equation} %
Note that the forms of policy parameterization for \eqref{eq:policy-parameterization} can be very flexible, such as linear mapping, polynomials, kernels, or neural networks. As we will show below, it is known that a linear map is sufficient for many optimal and robust control problems of linear time-invariant (LTI) systems \citep{zhou1996robust}. Then, the policy optimization \eqref{eq:policy-control-new} becomes a problem that aims to find the best finite-dimensional policy parameters $\theta$. In particular, under the policy $u_t = \pi_\theta(\mathcal{H}_t)$, the performance measure \eqref{eq:performance-measure} becomes a function of the policy parameter $\theta$, which can be denoted as 
$$
J(\x,\u) = \lim_{T \to \infty}\, \mathbb{E}_{w_t} \left(\frac{1}{T}\sum_{t=0}^T c(x_t, u_t)\right) =: J(\theta).
$$
Also, we can explicitly incorporate a policy constraint $\theta \in \Theta$ that represents closed-loop stability and/or certain information constraints. Consequently, an abstract form of policy optimization in control is 
\begin{equation}
\begin{aligned} \label{eq:policy-optimization}
    \min_{\theta} \quad & J(\theta) \\
    \mathrm{subject~to}\quad &  \theta \in \Theta. 
\end{aligned} 
\end{equation}

Conceptually, it appears simple and flexible to use local search algorithms, such as policy gradient or its variants, to seek the ``best'' policy for \eqref{eq:policy-optimization}. Once the corresponding cost in \eqref{eq:policy-optimization} can be estimated from sampled trajectories, this policy optimization setup indeed is very amenable for data-driven design paradigms such as reinforcement learning \citep{recht2019tour}. 
One goal of this article is to highlight some \textit{rich}, yet \textit{complicated} and \textit{intriguing}, geometry in policy optimization \eqref{eq:policy-optimization}, including nonconvexity, potentially disconnected feasible domain $\Theta$, spurious stationary points of the cost $J$, symmetry, and smooth (Riemannian) manifold structures. Our focus will be on classic and iconic control tasks for linear time-invariant (LTI) systems, including stabilization, LQR, LQG, and  $\mathcal{H}_\infty$ robust control. These geometrical understandings will often provide insights for designing principled local search algorithms to solve \eqref{eq:policy-optimization}, such as policy gradient methods with global/local convergence guarantees \citep{fazel2018global,mohammadi2021convergence,hu2023toward}. Inspired by the rich geometry in \eqref{eq:policy-optimization}, we will further emphasize that a ``complete policy parameterization'' should come with an associated metric, capturing the inherent geometry, which may help improve the problem's conditioning \citep{kraisler2024output,talebi_riemannian_2022}.    


In the following, we will present three classical control instances in the form of \eqref{eq:policy-optimization}: one is the problem of Linear Quadratic Regulator (LQR) with full state measurements, one is the problem of Linear Quadratic Gaussian (LQG) control with partial output measurements, and the final one is the problem of $\mathcal{H}_\infty$ robust control with adversarial noises. These three problems are arguably the most fundamental problems in optimal and robust control \citep{zhou1996robust}. %












\subsubsection{Linear Quadratic Regulator (LQR)}


For the LQR problem, the system dynamics \eqref{eq:general-dynamics} read as 
\begin{equation} \label{eq:state-evolution}
    {x}_{t+1}= Ax_t+Bu_t+ w_t, \qquad y_t = C x_t.
\end{equation}
where $C=I$ is the identity matrix, $x_t \in \mathbb{R}^n, u_t \in \mathbb{R}^m$ are the system state and input, and $w_t$ is a discrete-time white-noise process with a stationary full-rank covariance matrix $\Sigma \succ 0$. In \eqref{eq:state-evolution}, we assume that the state is directly observed. 
Given performance weights $Q \succeq 0, R \succ 0$, the stage cost is defined as $c(x_t, u_t) = x_t^\transpose Q x_t + u_t^\transpose R u_t$, and the LQR problem reads as
\begin{equation} \label{eq:LQR-stochastic-noise}
\begin{aligned}
\min_{u_0, u_1, \ldots}\ \ &
\lim_{T \to \infty} \mathbb{E}\!\left[\frac{1}{2T}\sum_{t=0}^{T}
\left(x^\transpose_t Q x_t+ u^\transpose_t R u_t\right)
\right]
\\
\text{subject to}\ \ & \eqref{eq:state-evolution}, 
\end{aligned}
\end{equation}
where the control input $u_t$ is allowed to depend on the entire history $(u_0, \ldots, u_{t-1}, x_0, \ldots, x_{t})$. 

Note that the cost in \Cref{eq:LQR-stochastic-noise} is oblivious to any bounded initial condition $x_0$ as long as the policy is stabilizing. Alternatively, when the dynamics is noiseless but the initial condition is uncertain, we might be interested in minimizing the following objective instead 
\begin{equation} \label{eq:LQR-no-noise}
\begin{aligned}
\min_{u_0, u_1, \ldots}\ \ &
\mathbb{E}_{x_0}\!\left[\frac{1}{2}\sum_{t=0}^{\infty}
\left(x^\transpose_t Q x_t+ u^\transpose_t R u_t\right)
\right]
\\
\text{subject to}\ \ & \x_{t+1} = A x_t + B u_t, 
\end{aligned}
\end{equation}
where $x_0$ is drawn from a distribution with covariance $\Sigma \succ 0$. We will see later that both of the problems in \Cref{eq:LQR-stochastic-noise} and \Cref{eq:LQR-no-noise} essentially amount to the same policy optimization problem.

Without loss of generality, for both  \eqref{eq:LQR-stochastic-noise} and \eqref{eq:LQR-no-noise}, we can parameterize the LQR policy as a linear mapping as  $u_t = Kx_t, K \in \mathbb{R}^{m \times n}$. Then, the set of stabilizing static state-feedback policies is  
\begin{equation} \label{eq:static-stabilizing-policies}
\mathcal{S} = \{K \in \mathbb{R}^{m \times n}: \rho(A+BK) < 1\}.
\end{equation}
where $\rho(\cdot)$ denotes the spectral radius of a square matrix. Let $J_{\texttt{LQR}}(K)\colon\mathcal{S}\rightarrow\mathbb{R}$ denote the function mapping a policy $K \in \mathcal{S} $ to its corresponding LQR cost~\eqref{eq:LQR-stochastic-noise} or \eqref{eq:LQR-no-noise}. Then, the policy optimization formulation \eqref{eq:policy-optimization} for LQR becomes 
\begin{equation}
\begin{aligned} \label{eq:LQR-policy-optimization}
    \min_{K} \quad & J_{\texttt{LQR}}(K) \\
    \mathrm{subject~to}\quad &  K \in \mathcal{S}. 
\end{aligned} 
\end{equation}





\subsubsection{Linear Quadratic Gaussian (LQG) Control}

We here specify the general optimal control problem \eqref{eq:general-optimal-control-new} in the context of LTI systems with partial observation. In particular, the dynamics \eqref{eq:general-dynamics} become a partially observed LTI system
\begin{equation} \label{eq:dynamics_discrete}
    \begin{aligned}
        x_{t+1} &= A x_t + B u_t + w_t, \\
        y_t &= Cx_t + v_t, 
    \end{aligned}
\end{equation}
where $x_t \in \mathbb{R}^n, u_t \in \mathbb{R}^m, y_t \in \mathbb{R}^p$ are the system state, input, and output measurement at time $t$, and $w_t \sim \mathcal{N}(0, W), v_t \sim \mathcal{N}(0, V)$ are Gaussian process and measurement noises, respectively.  It is assumed that the covariance matrices satisfy $W \succeq 0, V \succ 0$.
Given performance weight matrices $Q \succeq 0, R \succ 0$, the problem \eqref{eq:general-optimal-control-new}  for the LQG control is in the following form  
\begin{equation}~\label{eq:LQG_discrete}
    \begin{aligned}
        \min_{u_0,u_1, \ldots} &\quad \lim_{T \rightarrow \infty} \mathbb{E} \left[ \frac{1}{T} \sum_{t=1}^T\!\left(x_t^\transpose Q x_t + u_t^\transpose R u_t\right) \right] \\
        \text{subject to} &\quad~\eqref{eq:dynamics_discrete}. 
    \end{aligned}
\end{equation}
The control input $u_t$ at time $t$ is allowed to depend on the history $(u_0, \ldots, u_{t-1}, y_0, \ldots, y_{t-1})$. 


We consider a standard dynamic policy with the following parameterization 
\begin{equation} \label{eq:controller_discrete}
    \begin{aligned}
        \xi_{t+1} &= A_{\mK} \xi_t + B_{\mK} y_t, \\
        u_t &= C_{\mK} \xi_{t},
    \end{aligned}
\end{equation}
where $\xi_t \in \mathbb{R}^q$ is the policy internal state at time $t$, and policy parameters $(A_{\mK},B_{\mK},C_{\mK}) \in \mathbb{R}^{q \times q} \times \mathbb{R}^{q \times p} \times \mathbb{R}^{m \times q}$ specify the policy dynamics. If $q = n$, we refer to \eqref{eq:controller_discrete} as a \textit{full-order} dynamic policy; if $q < n$, it is called a \textit{reduced-order} dynamic policy. In this survey, we will mostly focus on the case $q = n$ since it is known that full-order dynamic policies contain the globally optimal solution to \eqref{eq:LQG_discrete} \citep{zhou1996robust}. 
Combining~\eqref{eq:controller_discrete} with~\eqref{eq:dynamics_discrete} leads to the closed-loop system below 
\begin{equation}\label{eq:closed_loop_system}
\begin{aligned}
   \begin{bmatrix} x_{t+1} \\ \xi_{t+1} \end{bmatrix} &= \begin{bmatrix}
    A & BC_{\mK} \\
    B_{\mK}C & A_{\mK}
    \end{bmatrix} \begin{bmatrix} x_t \\ \xi_t \end{bmatrix}  +  \begin{bmatrix} I & 0 \\ 0 & B_{\mK}  \end{bmatrix}\begin{bmatrix} w_t \\ v_t \end{bmatrix} \\
    \begin{bmatrix} y_t \\ u_t \end{bmatrix}& = \begin{bmatrix} C & 0 \\ 0& C_{\mK} \end{bmatrix} \begin{bmatrix} x_t \\ \xi_t \end{bmatrix} + \begin{bmatrix} v_t \\0 \end{bmatrix}.
\end{aligned}
\end{equation}
The set of stabilizing controllers with order $q \in \mathbb{N}$ is defined as %
\begin{equation} \label{eq:internallystabilizing}
    \mathcal{C}_{q} := \left\{
    \left.\mK=\begin{bmatrix}
    0_{m\times p} & C_{\mK} \\
    B_{\mK} & A_{\mK}
    \end{bmatrix}
    \in \mathbb{R}^{(m+q) \times (p+q)} \right|\;  \rho\left(\begin{bmatrix}
    A & BC_{\mK} \\
    B_{\mK}C & A_{\mK}
    \end{bmatrix}\right) < 1\right\},
\end{equation}
Let $J_{_{\texttt{LQG}},q}(\mK)\colon\mathcal{C}_q\rightarrow\mathbb{R}$ denote the function that maps a parameterized dynamical controller in $\mathcal{C}_q$ to its corresponding LQG cost for each $q\in\mathbb{N}$. Given the dimension $n$ of the plant's state variable, the LQG problem~\eqref{eq:LQG_discrete} can be reformulated into a constrained optimization problem:
\begin{equation} \label{eq:LQG_policy-optimization}
    \begin{aligned}
        \min_{\mK} \quad &J{_{\texttt{LQG},n}}(\mK) \\
        \text{subject to} \quad& \mK \in \mathcal{C}_n. 
    \end{aligned}
\end{equation}
Throughout this survey, we make the standard assumption that $(A,B)$ is stabilizable and $(C,A)$ is detectable for the LTI system \eqref{eq:dynamics_discrete}, so that $\mathcal{C}_n$ is nonempty.  



\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width = 0.24\textwidth]{figures/3d_policy_11.png}}
    \subfigure[]{\includegraphics[width = 0.24\textwidth]{figures/3d_policy_21.png}}
    \subfigure[]{\includegraphics[width = 0.24\textwidth]{figures/3d_policy_12.png}}
    \subfigure[]{\includegraphics[width = 0.24\textwidth]{figures/3d_policy_22.png}}
    \caption{The nonconvex (4-D) set of stabilizing policies $\stableK$ in \eqref{eq:static-stabilizing-policies} with $A = \begin{bmatrix}1 &1\\0 & 1\end{bmatrix}$ and $B = \begin{bmatrix}0 &1\\1 & 0\end{bmatrix}$. We illustrate the intersection of $\stableK$ with the affine subspaces that are passing through $K_0 = -\begin{bmatrix}0 &0.8\\0.9 & 0.9\end{bmatrix}$ and are orthogonal to the direction $E$ where  
    (a) $E = \begin{bmatrix}1 &0\\0 & 0\end{bmatrix}$, (b) $E = \begin{bmatrix}0 &1\\0 & 0\end{bmatrix}$, 
    (c) $E = \begin{bmatrix}0 &0\\1 & 0\end{bmatrix}$, and (d) $E = \begin{bmatrix}0 &0\\0 & 1\end{bmatrix}$. \shahriar{improve the labels... the color is horrible.}}
    \label{fig:LQR-simple}
\end{figure}


\subsubsection{$\mathcal{H}_\infty$ robust control}

When the disturbance $w_t$ in system \eqref{eq:state-evolution} is not stochastic but adversarial with bounded energy, e.g., $\|w\|_{L_2}^2 \coloneqq \sum_{t=0}^\infty w_t^\transpose w_t \leq 1$, one typical control goal is to design a sequence of control inputs $u_t$ that improve the worst-case performance (i.e., the closed-loop robustness). In classical control, the worst-case performance is typically measured by an $\mathcal{H}_\infty$ norm of a certain closed-loop channel, and thus this problem is known as $\mathcal{H}_\infty$ robust control.

The worst-case performance when $w_t$ has bounded energy less than or equal to 1 is measured~by 
\begin{equation} \label{eq:Hinf-cost-def}
    {J}_{\infty} := \sup_{\|w\|^2_{L_2} \leq 1} \sum_{t=0}^\infty \left(x_t^\transpose Q x_t + u_t^\transpose R u_t\right), 
\end{equation}
where $Q \succeq 0, R \succ 0$ are given weights.  
The (state-feedback) $\mathcal{H}_\infty$ robust control is formulated as
\begin{equation*} %
    \begin{aligned}
        \min_{u_0, u_1, \ldots} \quad & {J}_{\infty} \\
        \text{subject to} \quad & ~\eqref{eq:state-evolution} \text{ and }
        x(0)=0,
    \end{aligned}
\end{equation*}

where similarly $u_t$ is allowed to depend on the entire history $(u_0, \ldots, u_{t-1}, x_0, \ldots, x_{t})$. Without loss of generality, we can parameterize the $\mathcal{H}_\infty$ policy as a linear mapping $u_t = Kx_t, K \in \mathbb{R}^{m \times n}$ \citep{zhou1988algebraic}, and the set of stabilizing policies is the same as \eqref{eq:static-stabilizing-policies}. 

Let $J_\infty(K)\colon\mathcal{S}\rightarrow\mathbb{R}$ denote the function mapping a policy $K \in \mathcal{S} $ to its corresponding worst performance~\eqref{eq:Hinf-cost-def}. Then, the policy optimization formulation \eqref{eq:policy-optimization} for $\mathcal{H}_\infty$ robust control becomes 
\begin{equation}
\begin{aligned} \label{eq:Hinf-policy-optimization}
    \min_{K} \quad & J_\infty(K) \\
    \mathrm{subject~to}\quad &  K \in \mathcal{S}. 
\end{aligned} 
\end{equation}
This problem \eqref{eq:Hinf-policy-optimization} is a state-feedback $\mathcal{H}_\infty$ control, where we can use a linear static policy with no loss of generality \citep{zhou1988algebraic}. As the partially observed LTI system \eqref{eq:dynamics_discrete} where the state $x_t$ is not directly measured, we can consider the general output-feedback $\mathcal{H}_\infty$ control, in which a dynamic policy similar to \eqref{eq:controller_discrete} is needed \citep{zhou1996robust}. At the time of writing, geometrical properties for output-feedback $\mathcal{H}_\infty$ control are under active investigation; see e.g., \citep{zheng2023benign,tang2023global,guo2024complexity}. We will not pursue the details here.     


\subsection{Towards (non-convex) geometry and Riemannian manifold structures} \label{subsection:geometry-manifold}

\vspace{5mm}
\yang{This subsection can be expanded a little. We can incorporate some discussions/points from the introduction here. We can make those discussions more concrete.}
\vspace{5mm}

The general policy optimization \eqref{eq:policy-optimization} and its specialized forms for LQR \eqref{eq:LQR-policy-optimization}, for LQG \eqref{eq:LQG_policy-optimization} and for $\mathcal{H}_\infty$ control \eqref{eq:Hinf-policy-optimization} are all in general non-convex in the space of policy parameters. Indeed, it is easy to find explicit examples to show that both the domains, i.e., stabilizing static policies $K \in \mathcal{S}$ and dynamic policies $\mK \in \mathcal{C}_n$, and the corresponding cost functions, i.e., LQR/LQG/$\mathcal{H}_\infty$ costs, are non-convex; see \Cref{fig:LQR-simple} for an illustration. We will detail more topological properties and Riemannian manifold structures of the domain in \Cref{section:stablizing-policies} and of the cost functions in \Cref{section:LQ-performance}.   

\shahriar{I'll update this opening...} The policy parameterization approach for optimal control \eqref{eq:general-optimal-control-new} brings the rich geometry in \eqref{eq:policy-optimization}. One main argument in this survey is to bring a ``complete parameterization'' by utilizing proper Riemannian manifold structures that capture the geometry in \eqref{eq:policy-optimization}, which may improve the problem's conditioning.    
In the case of LQR \eqref{eq:LQR-policy-optimization}, a complete parametrization may be a Riemannian manifold $(\mathcal{S}, g)$ where $g$ is a Riemannian metric that captures the geometry of \eqref{eq:LQR-policy-optimization}. This explicit Riemannian metric $g$ will be studied later in detail in \Cref{subsection:static-stabilizing-policies}, and the norm $\|K\|_g$ of a policy parameter $K \in \mathcal{S}$ in this Riemannian metric\footnote{The quantity $\|K\|_g$ should be interpreted under the so-called \textit{usual identification} of the tangent bundle.} is equivalent to the ``average input energy'' of the closed-loop system with the policy $u_t = Kx$ --- the norm of $K$ in the normal Euclidean metric does not provide such relevance. 

As for dynamic policies in the case of LQG \eqref{eq:LQG_policy-optimization}, there exists an inherent \textit{symmetry} for both $\mathcal{C}_n$ and $J_n(\mK)$, arising from standard similarity transformations in control. A similarity transformation reflects a coordinate change for the internal state of policy \eqref{eq:controller_discrete}. In particular, given any invertible matrix $T \in \mathrm{GL}_n$, a transformation $\mK = (A_\mK, B_\mK, C_\mK) \to \hat{\mK} = (T A_\mK T^{-1}, TB_\mK, C_\mK T^{-1})$ preserves both closed-loop stability and closed-loop LQG performance, i.e., we have $\mK \in \mathcal{C}_n \Leftrightarrow \hat{\mK} \in \mathcal{C}_n$ and $J_n(\mK) = J_n(\hat{\mK})$. Indeed, we can define an \textit{orbit} for each $\mK \in \mathcal{C}_n$, over which the closed-loop LQG performance remains constant. However, the local geometry around each point can be drastically different due to the effect of coordinate change by $T \in \mathrm{GL}_n$, that is $\nabla J_n(\mK)$ can be very different from $\nabla J_n(\hat{\mK})$ \cite[Lemma 10]{tang2023analysis}.  For example,  it is possible that choosing $T$ with $\|T\|_{\mathrm{F}} \gg 1$ may result in $\|\nabla J_n(\hat{\mK})\|_{\mathrm{F}} \gg 1$ even $\|\nabla J_n({\mK})\|_{\mathrm{F}}$ is not large. As a result, this ill-conditioning of the internal coordinates may result in numerical instability for direct policy optimization algorithms. It will be more beneficial to explicitly incorporate this symmetry as proper Riemannian manifold structures during the algorithm design of local policy search \citep{kraisler2024output}. 





\vspace{20mm}

\textbf{Rest of the points that wanna make here:}
\begin{itemize}
    \item When is policy optimization a good idea?, when it is not?
    \item  PO is a more direct bridge between optimization and control. Why this can be tricky?
    \item  We can talk about convex reparameterization a bit which might not always be known (like Youla and LMI formulations in presence of general constraints) which may be limiting; on the other hand, direct PO optimization can be though of as a general formulation and when equipped with appropriate geometry can be powerful.
    \item Almost all convex parameterizations rely on the underlying system model, which may not be available or poorly understood.
    \item Why do we look for convexity (in the Euclidean sense) for direct policy parameterization? What does it mean to do convex combination of two stabilizing policies $K_1$ and $K_2$? In fact, this is purely an artifact of our direct parameterization and choice of coordinate frame.  One remedy for this can be to allow for general Riemannian metrics to describe the relevant geometry; for instance, what should a ``convex combination of policies'' look like! This can certainly be a POV to entice the reader.
\end{itemize}







==> policy-optimization.tex <==
\section{Policy Optimization in Control: Role of Parameterization} \label{parameterization}

Optimal control offers a principled use of feedback to influence and steer the behavior of a dynamical system in order to achieve a desired goal, while minimizing a certain performance cost. Let us consider a discrete-time dynamical system:
\begin{equation}\label{eq:system-dynamics}
         x_{t+1} = f(x_t,u_t,w_t), \quad y_t = h(x_t,w_t),
\end{equation} 
where $x_t \in \mathbb{R}^n$ is the system state, $u_t \in \mathbb{R}^m$ is the control input, and $y_t \in \mathbb{R}^p$ is the system measurement. We refer to $w_t$ as the exogenous signal,
representing for example, unmodeled dynamics, stochastic noise, or disturbances.
At each time step $t$, we use $l(x_t,u_t)$ to denote the stage cost as a function of the current state and input. The goal of infinite-horizon optimal control is to choose $\mathbf{u}=(u_0,u_1,\ldots)$ to minimize an accumulated cost over the infinite time horizon. 
More formally, we define the $T$-stage accumulated cost as
\begin{subequations}\label{eq:ave-inf-hor-cost}
    \begin{align}
        J_{T}(\mathbf{u}, \mathbf{w}, x_0) \coloneqq  \sum_{t=0}^T l(x_t,u_t),    
    \end{align}
\end{subequations}
where $\mathbf{w}=(w_0,w_1,\ldots)$. The cost (\ref{eq:ave-inf-hor-cost}) highlights that the state trajectory built into the definition of $J$ depends on the control input $\mathbf{u}$, the exogenous input $\mathbf{w}$, and initial state $x_0$.
Often $\mathbf{w}$ and $x_0$ are modeled either stochastically or deterministically, and the performance of the closed-loop system is measured based on the corresponding average or worst case performance. Examples of such infinite-horizon control performance measures include,
\begin{subequations}\label{eq:single-param-ave-inf-hor-cost}
    \begin{align}
        J_2(\mathbf{u})  &:= \lim_{T \to \infty} \mathbb{E}_{x_0}\;  J_T(\mathbf{u}, \mathbf{0}, x_0), \label{eq:inf-hor-no-noise}\\
        J_2(\mathbf{u}) &:= \lim_{T \to \infty} \mathbb{E}_{\mathbf{w},x_0} \;\frac{1}{T} J_T(\mathbf{u},\mathbf{w}, x_0),\label{eq:inf-hor-noise}\\
        J_\infty(\mathbf{u}) &:=\sup_{\|\mathbf{w}\|_{\ell_2} \leq 1}  %
        \lim_{T \to \infty} \mathbb{E}_{x_0} J_T(\mathbf{u},\mathbf{w}, x_0),\label{eq:robust-cost}
    \end{align}
\end{subequations}
where \Cref{eq:inf-hor-no-noise} presumes no exogenous input (as such we denote $\mathbf{0}=(0,0, \ldots)$),  %
\cref{eq:inf-hor-noise} considers with stochastic exogenous input (by expectation with respect to statistical properties of the exogenous input and initial condition), and \cref{eq:robust-cost} considers adversarial exogenous input (by taking the worst case performance with respect to a normalized uncertainty). Here, $\ell_2$ denotes the space of square-integrable sequences endowed with its ``natural'' 2-norm $\|. \|_{\ell_2}$, and the notation $J_2$ and $J_\infty$ are chosen to highlight their corresponding system norm interpretations in $\mathcal{H}_2$ and $\mathcal{H}_\infty$ synthesis.
In the special case of linear dynamics and quadratic stage cost, performance measures \cref{eq:inf-hor-no-noise} and \cref{eq:inf-hor-noise} with stationary exogenous noise are essentially equivalent, justifying their analogous notation.
We will also denote a general performance measure as $J$.



\subsection{Policy Parameterization for Closed-loop Optimal Control}

Instead of optimizing over the input sequence $\mathbf{u}$ in (\ref{eq:single-param-ave-inf-hor-cost}), which we refer to as the \textit{optimal open-loop control design}, we consider instead
optimizing over a class of \textit{feedback policies} that act
on the system history $\mathcal{H}_t := (u_{0:t-1}, y_{0:t}) \in \mathbb{R}^{m \times t} \times \mathbb{R}^{p \times (t + 1)}$, where $u_{0:t-1} := (u_0,u_1,\ldots,u_{t-1})$ and similarly for $y_{0:t}$. As such \textit{feedback} or \textit{closed-loop policy} at time $t$, denoted by $\pi_t:\mathbb{R}^{m \times t} \times \mathbb{R}^{p \times (t + 1)} \to \mathbb{R}^m$, is a measurable function that maps the system history $\mathcal{H}_t$ at time $t$ to a control input $u_t$. We can alternatively define $\pi_t(\mathcal{H}_t)$ to be a distribution and set $u_t \sim \pi_t(\mathcal{H}_t)$.\footnote{In this case, we would have to slightly augment (\ref{eq:single-param-ave-inf-hor-cost}).} We will call $\pi=(\pi_0,\pi_1,\ldots)$ the feedback policy;
for brevity, we will often write $\pi(\mathcal{H}_t):=\pi_t(\mathcal{H}_t)$. 
Let $\Pi$ be the infinite-dimensional vector space of all such feedback policies $\pi(\cdot)$. 
Then, the optimal closed-loop policy problem reads as 
\begin{subequations}\label{eq:closed-loop-policy-prob}
    \begin{align}
        \min_{\pi \in \Pi} \quad & \ J(\mathbf{u}) \\
        \text{subject to} \quad &(\ref{eq:system-dynamics}),\;  
        u_t = \pi(\mathcal{H}_t), %
    \end{align}
\end{subequations} where $J(\mathbf{u})$ can take any of the forms in (\ref{eq:single-param-ave-inf-hor-cost}). Throughout this work, the decision variables are the policies $\pi(\cdot) \in \Pi$.

Since it is non-trivial to optimize directly over this space $\Pi$, the so-called ``policy parameterization'' approach is to parameterize a subset of $\Pi$ with a finite set of parameters $\theta \in \Theta \subset \mathbb{R}^{n_p}$. That way, our parameterized family of policies $\{\pi_\theta(\cdot)\}_{\theta \in \Theta} \subset \Pi$ is finite-dimensional. Note that policy parameterization is rather flexible, as it can represent linear dynamical systems, polynomials, kernels, or neural networks. In some important cases, one can restrict the class of policies under consideration without loss of generality. For instance, it is known that static/dynamic ``linear policies'' are sufficient for optimal and robust control problems posed for linear time-invariant (LTI) systems~\citep{zhou1996robust}. With policy parameterization, \eqref{eq:closed-loop-policy-prob} is reduced to an optimal closed-loop parameterized policy problem that aims to find the best \textit{parameterized} policy~$\pi_\theta$:

\begin{equation} \label{eq:closed-loop-param-policy-prob}
    \min_{\theta \in \Theta}  J(\theta) := J(\pi_{\theta}(\mathcal{H})), 
\end{equation} 
where $\pi_{\theta}(\mathcal{H})$ denotes the input signal obtained as $\mathbf{u} = (\pi_\theta(\mathcal{H}_0), \pi_\theta(\mathcal{H}_1), \dots)$. If $\pi^*$ solves (\ref{eq:closed-loop-policy-prob}) and $\theta^*$ solves (\ref{eq:closed-loop-param-policy-prob}) then it should be remarked $J(\pi^*) \leq J(\pi_{\theta^*})$, with equality if and only if the parameterization is ``rich enough,'' e.g., linear static/dynamic feedback policies for LQR/LQG problems.
Further, we can explicitly incorporate a policy constraint on $\Theta$ that represents closed-loop stability or constraints 
on the information structure required for control synthesis.

Conceptually, it appears simple and flexible to use local search algorithms, such as policy gradient or its variants, to seek the ``best'' policy in \eqref{eq:closed-loop-param-policy-prob}. Once the corresponding cost in \eqref{eq:closed-loop-param-policy-prob} can be estimated from sampled trajectories, this policy optimization setup indeed is very amenable for data-driven design paradigms such as reinforcement learning \citep{recht2019tour}. 
One goal of this article is to highlight some \textit{rich} and \textit{intriguing}, geometry in policy optimization \eqref{eq:closed-loop-param-policy-prob}, including nonconvexity, potentially disconnected feasible domain $\Theta$, spurious stationary points of the cost $J$, symmetry, and smooth (Riemannian) manifold structures. Our focus will be on classic control tasks for LTI systems including LQR, LQG, and  $\mathcal{H}_\infty$ robust control. These geometrical understandings will often provide insights for designing principled local search algorithms to solve \eqref{eq:closed-loop-param-policy-prob}, such as policy gradient methods with global/local convergence guarantees \citep{fazel2018global,bu_lqr_2019,mohammadi2021convergence,hu2023toward}. Inspired by the rich geometry in \eqref{eq:closed-loop-param-policy-prob}, we will further emphasize that a ``complete policy parameterization'' should come with an associated metric, capturing the inherent geometry, which may help improve the problem's conditioning \citep{talebi_riemannian_2022,kraisler2024output}.   




\subsubsection{LQR under Static State-feedback Policies}


For the LQR problem, the system dynamics \eqref{eq:system-dynamics} read as 
\begin{equation} \label{eq:state-evolution}
    {x}_{t+1}= Ax_t+Bu_t+ w_t, \qquad y_t = x_t,
\end{equation} 
where the process noise is white and Gaussian $w_t \sim \mathcal{N}(0, \Sigma)$ for some $\Sigma \succ 0$.
Since the state is directly observed, the system history takes the form $\mathcal{H}_t = (u_{0:t-1}, x_{0:t})$. Given the performance weighting matrices $Q \succeq 0, R \succ 0$, (\ref{eq:closed-loop-policy-prob}) reduces to the optimal LQR problem:
\begin{subequations}\label{eq:LQR-noise}
    \begin{align}
    \min_{\pi \in \Pi} \quad &J_{\texttt{LQR}}(\mathbf{u}) \coloneqq \lim_{T \to \infty} \mathbb{E}_{\mathbf{w},x_0} \; \frac{1}{T}J_T(\mathbf{u},\mathbf{w}, x_0) \\
    \text{subject to}\quad &(\ref{eq:state-evolution}), \; u_t = \pi(\mathcal{H}_t)
    \end{align} 
\end{subequations} where we are using the stage cost $l(x_t,u_t)=\frac{1}{2}(x_t^TQx_t + u_t^TRu_t)$. 
Note that the cost in \Cref{eq:LQR-noise} will be oblivious to any bounded initial condition $x_0$ as long as the policy is stabilizing, and the Gaussian assumption on noise is for simplicity.

Alternatively, when the dynamics is noiseless but the initial condition is uncertain, we might be interested in minimizing the following objective instead 
\begin{subequations}\label{eq:LQR-noiseless}
    \begin{align}
        \min_{\pi \in \Pi} \quad &J_{\texttt{LQR}}(\mathbf{u}) \coloneqq \lim_{T \to \infty} \mathbb{E}_{x_0}\;  J_T(\mathbf{u}, \mathbf{0}, x_0) \\
        \text{subject to} \quad &(\ref{eq:state-evolution}), \; u_t = \pi(\mathcal{H}_t)
    \end{align}
\end{subequations} where $x_0$ is drawn from a distribution with covariance $\Sigma \succ 0$. We will see later that both of the problems in (\ref{eq:LQR-noise}) and (\ref{eq:LQR-noiseless}) essentially amount to the same policy optimization problem. 

A remarkable property of the closed-loop optimal LQR problem is that the optimal policy $\pi^*$, when it exists, is linear in the state and depends only on the current state. That is, $\pi^*(\mathcal{H}_t) = \pi^*(x_t) = K x_t$ for some $K \in \mathbb{R}^{m \times n}$ \citep{anderson_optimal_2007}.
Inspired by this property, for both  \eqref{eq:LQR-noise} and \eqref{eq:LQR-noiseless}, we can parameterize the LQR policy as a linear mapping $x_t \mapsto u_t = Kx_t$ and referred to as policy $K$ for simplicity. Then, the set of static stabilizing state-feedback policies is  
\begin{equation} \label{eq:static-stabilizing-policies}
    \Theta := \mathcal{S} = \{K \in \mathbb{R}^{m \times n}: \rho(A+BK) < 1\}.
\end{equation} where $\rho(\cdot)$ denotes the spectral radius of a square matrix. Following (\ref{eq:closed-loop-param-policy-prob}), we can define $J_{\texttt{LQR}}$ over $\mathcal{S}$, where $J_{\texttt{LQR}}(K)$ corresponds to the objective in either~\eqref{eq:LQR-noise} or \eqref{eq:LQR-noiseless}. Our parameterized policy family will be $\{\pi_K\}_{K \in \mathcal{S}}$ with $\pi_K(\mathcal{H}_t) := K x_t$.
Lastly, the optimal LQR policy problem becomes 
\begin{equation}
\begin{aligned} \label{eq:LQR-policy-optimization}
    \min_{K} \quad & J_{\texttt{LQR}}(K) \\
    \mathrm{subject~to}\quad &  K \in \mathcal{S}. 
\end{aligned} 
\end{equation}
For well-posedness of the problem, we assume that the pair $(A,B)$ is stabilizable so $\stableK$ is non-empty. 

\subsubsection{LQG under Dynamic Output-feedback Policies}\label{subsubsect:LQG}

We here specify the general closed-loop optimal policy problem \eqref{eq:closed-loop-policy-prob} in the context of LTI systems with partial observation:
\begin{equation} \label{eq:dynamics_discrete}
    \begin{aligned}
        x_{t+1} = A x_t + B u_t + w_t, \qquad  
        y_t = Cx_t + v_t, 
    \end{aligned}
\end{equation}
where $x_t \in \mathbb{R}^n, u_t \in \mathbb{R}^m, y_t \in \mathbb{R}^p$ are the system state, input, and output measurement at time $t$, and $w_t \sim \mathcal{N}(0, W), v_t \sim \mathcal{N}(0, V)$ are Gaussian process and measurement noise signals, respectively.  It is assumed that the covariance matrices satisfy $W \succeq 0, V \succ 0$.
Given performance weight matrices $Q \succeq 0, R \succ 0$, the optimal LQG problem becomes,
\begin{subequations}\label{LQG-policy-problem}
    \begin{align}
        \min_{\pi \in \Pi} \quad &J_{\texttt{LQG}}(\mathbf{u}) \coloneqq \lim_{T \to \infty} \mathbb{E}_{\mathbf{w},x_0} \; \frac{1}{T} J_T(\mathbf{u},\mathbf{w}, x_0) \\ \label{eq:LQG-cost}
        \text{subject~to} \quad &(\ref{eq:dynamics_discrete}), \; u_t = \pi(\mathcal{H}_t)
    \end{align}
\end{subequations} where $\mathbf{w} := ((w_t,v_t))_{t=0}^\infty$. It should be noted that the difference between the optimal closed-loop policy problems (\ref{LQG-policy-problem}) and (\ref{eq:LQR-noise}) is the policies have to only depend on the output-feedback $\mathcal{H}_t = (u_{0:t-1},y_{0:t-1})$ versus state-feedback $(u_{0:t-1},x_{0:t})$, respectively. 

Next, we construct a family of policies, referred to as \textit{dynamic policies}, parameterized by an LTI system,
\begin{equation} \label{eq:controller_discrete}
    \begin{aligned}
        \xi_{t+1} = A_{\mK} \xi_t + B_{\mK} y_t, \quad 
        u_t = C_{\mK} \xi_{t}, 
    \end{aligned}
\end{equation}
where $\xi_t \in \mathbb{R}^q$ is the policy internal state at time $t$, and policy parameters $(A_{\mK},B_{\mK},C_{\mK}) \in \mathbb{R}^{q \times q} \times \mathbb{R}^{q \times p} \times \mathbb{R}^{m \times q}$ specify the policy dynamics. If $q = n$, we refer to \eqref{eq:controller_discrete} as a \textit{full-order} dynamic policy; if $q < n$, it is called a \textit{reduced-order} dynamic policy. In this survey, we will mostly focus on the case $q = n$ since it is known that full-order dynamic policies contain a globally optimal solution to the closed-loop optimal policy problem \eqref{LQG-policy-problem} \citep{zhou1996robust}. 
Therefore, combining~\eqref{eq:controller_discrete} with~\eqref{eq:dynamics_discrete} leads to the augmented closed-loop system,
\begin{equation}\label{eq:closed_loop_system}
\begin{aligned}
   \begin{bmatrix} x_{t+1} \\ \xi_{t+1} \end{bmatrix} &= \begin{bmatrix}
    A & BC_{\mK} \\
    B_{\mK}C & A_{\mK}
    \end{bmatrix} \begin{bmatrix} x_t \\ \xi_t \end{bmatrix}  +  \begin{bmatrix} I & 0 \\ 0 & B_{\mK}  \end{bmatrix}\begin{bmatrix} w_t \\ v_t \end{bmatrix} \\
    \begin{bmatrix} y_t \\ u_t \end{bmatrix}& = \begin{bmatrix} C & 0 \\ 0& C_{\mK} \end{bmatrix} \begin{bmatrix} x_t \\ \xi_t \end{bmatrix} + \begin{bmatrix} v_t \\0 \end{bmatrix}.
\end{aligned}
\end{equation}
The set of stabilizing controllers with order $q \in \mathbb{N}$ is now defined as, %
\begin{equation} \label{eq:internallystabilizing}
    \Theta := \mathcal{C}_{q} = \left\{
    \left.\mK=\begin{bmatrix}
    0_{m\times p} & C_{\mK} \\
    B_{\mK} & A_{\mK}
    \end{bmatrix}
    \in \mathbb{R}^{(m+q) \times (p+q)} \right|\;  \rho\left(\begin{bmatrix}
    A & BC_{\mK} \\
    B_{\mK}C & A_{\mK}
    \end{bmatrix}\right) < 1\right\}.
\end{equation}
Then, any such $\mK \in \mathcal{C}_q$ determines a dynamic policy $\pi_{\mK}$ with $\pi_{\mK}(\mathcal{H}_t) := \sum_{i=1}^t C_{\mK} A_{\mK}^{i - 1}B_{\mK} y_{t - i }$, where we set $\xi_0 = 0$.
Following the parameterization in (\ref{eq:closed-loop-param-policy-prob}), given the system plant dimension $n$, the policy optimization for LQG control becomes
\begin{equation}
\begin{aligned} \label{eq:LQG_policy-optimization}
    \min_{\mK} \quad & J_{\texttt{LQG}}(\mK) \\
    \mathrm{subject~to}\quad &  \mK \in \mathcal{C}_n. 
\end{aligned} 
\end{equation}
Throughout this survey, we make the standard assumption that $(A,B)$ is stabilizable and $(C,A)$ is detectable for the LTI system \eqref{eq:dynamics_discrete}, so that $\mathcal{C}_n$ is nonempty.  




\begin{figure}[t]
    \centering
    \includegraphics[width=.4\textwidth]{figures/static_controller_manifold.pdf}
    \caption{The non-convex set of stabilizing static state-feedback polices $\stableK$ for $A = \begin{bmatrix} 0 & 1 & 0 \\ 0 & 0 & 1 \\ 0 & 0 & 0\end{bmatrix}$ and 
$B = \begin{bmatrix} 0 \\ 0 \\ 1\end{bmatrix}$. Note that the non-convex shape extends further towards negative direction of $K_2$ axis.
}
    \label{fig:LQR-simple}
\end{figure}

\subsubsection{$\mathcal{H}_\infty$-norm under Static State-feedback Policies}\label{subsubsect:state-feedback-robust-control}

The performance (\ref{eq:robust-cost}) characterized the worst case performance against the disturbance $w_t$ that is not stochastic but adversarial with bounded energy, which coincides with the $\mathcal{H}_\infty$ norm of a closed-loop transfer function. Considering the same dynamics in \Cref{eq:state-evolution}, then \Cref{eq:closed-loop-policy-prob} reduces to the $\mathcal{H}_\infty$ robust control problem: 
\begin{equation*} %
    \begin{aligned}
        \min_{\pi \in \Pi} \quad & J_\infty(\mathbf{u}):= \sup_{\|\mathbf{w}\|_{l_2} \leq 1} \lim_{T \to \infty} J_T(\mathbf{u}, \mathbf{w}, 0) \\
        \text{subject to} \quad & ~\eqref{eq:state-evolution}, \;
        u_t = \pi(\mathcal{H}_t),
    \end{aligned}
\end{equation*}
where we have assumed $x_0=0$ for simplicity.
Following (\ref{eq:closed-loop-param-policy-prob}) and by considering the same parameterization as LQR, we can equivalently express $J_\infty$ instead as a function on the set of static stabilizing policies $\mathcal{S}$, and thus the $\mathcal{H}_\infty$-robust policy problem becomes,
\begin{equation}
\begin{aligned} \label{eq:Hinf-policy-optimization}
    \min_{K} \quad & J_{\infty}(K) \\
    \mathrm{subject~to}\quad &  K \in \mathcal{S}. 
\end{aligned} 
\end{equation}
Note that \cref{eq:Hinf-policy-optimization} is the state-feedback $\mathcal{H}_\infty$ control based on dynamics in \Cref{eq:state-evolution}, where the \textit{static linear} policy parameterization results in no loss of optimality \citep{zhou1988algebraic}. For the partially observed LTI system \eqref{eq:dynamics_discrete} where the state $x_t$ is not directly measured, we can consider the general output-feedback $\mathcal{H}_\infty$ control, in which a dynamic policy similar to \eqref{eq:controller_discrete} is required \citep{zhou1996robust}.   

\subsection{Towards Non-Convex Optimization and Riemannian Manifolds} \label{subsection:geometry-manifold}
\mehran{would it make sense that we remove this section as i think we dive into these topics in the subsequent sections anyways?}




\lina{connecting to a comment I put for theorem 3.2. We should add a definition for Riemannian manifold. This section may be the right place.} \shahriar{I agree with you Lina. My original intention of this section was just a smooth transition to next section, but How about moving some of the general definitions to this section?}
The general policy optimization %
\eqref{eq:closed-loop-param-policy-prob} 
and its specialized forms for LQR \eqref{eq:LQR-policy-optimization}, for LQG \eqref{eq:LQG_policy-optimization} and for $\mathcal{H}_\infty$ control \eqref{eq:Hinf-policy-optimization} are all in general \textit{non-convex} in the space of policy parameters; we refer to \cite{bu_topological_2021} for a complete characterization. \lina{It would be helpful to cite jingjing's paper here and say that readers can refer to [] for a complete characterization of ... }\shahriar{addressed.}. 
Indeed, it is easy to find explicit examples to show that both the domains, i.e., stabilizing static policies $K \in \mathcal{S}$ and dynamic policies $\mK \in \mathcal{C}_n$, and the corresponding cost functions, i.e., LQR/LQG/$\mathcal{H}_\infty$ costs, are non-convex; see \Cref{fig:LQR-simple} for an illustration.\spencer{can this paragraph be shortened to 2-3 sentences? I think it can}
We will detail more topological properties and Riemannian manifold structures of these domains in \S\ref{section:stablizing-policies} and of the cost functions in \S\ref{section:LQ-performance}.




One of the motivations of parameterizing policies as in \cref{eq:closed-loop-param-policy-prob} is to take advantage of optimization techniques to iteratively learn the optimal policy for these optimal control problem. Even though, these are, in general, non-convex problems and requires problem-specific treatment our aim is to keep up with Hilbert's advice on:
\begin{quote}
    The art of doing mathematics consists in finding that special case which contains all the germs of generality.
\end{quote}
Along this line, we show that the policy parameterization approach for these optimal control problems contains a rich geometry that can be captured by Riemannian geometric tools beyond the standard Euclidean optimization techniques. At the same time, one main argument in this survey is to bring a ``complete parameterization'' by equipping the domains of feasible policy parameters with relevant Riemannian manifold structures that capture the geometry in each of these problems. This not only enables us to incorporate general Riemannian optimization techniques but also allows for improving the problem's conditioning and devise more efficient algorithms.    
In order to provide a brief preview on this idea, we take a glance at the Riemannian geometries of LQR and LQG problems. 

\spencer{i dont see the need for these two paragraphs; all of this is already explained in detail in their respective sections}

Considering the case of LQR in \eqref{eq:LQR-policy-optimization}, a complete parametrization may be a Riemannian manifold $(\mathcal{S}, \tensor{\cdot}{\cdot}{}^\texttt{L})$ capturing the geometry of \eqref{eq:LQR-policy-optimization}. This explicit Riemannian metric $\tensor{\cdot}{\cdot}{}^\texttt{L}$ will be studied later in detail in \Cref{subsection:static-stabilizing-policies}, and the norm $\|K\|_{K}^2 = \tensor{K}{K}{K}^\texttt{L}$ \lina{is the subscript $K$ redundant?}\shahriar{For this to makes sense, the metric should be evaluated at the same policy $K$. I will make sure the notation is consistent at the next round.}of a policy parameter $K \in \mathcal{S}$ in this Riemannian metric\footnote{The quantity $\|K\|_{K}^2$ should be interpreted under the so-called \textit{usual identification} of the tangent bundle.\spencer{this doesnt make much sense to me.} \shahriar{I'm not sure whay the definition of ``usual identification'' is removed? otherwise this should be clear.} \spencer{my point is that, to me, $\|K\|_K$ is simply a consequence of the fact that $\stableK$ is an open set. im not convinced it has any mathematical meaning beyond this coincedence. i would need to see a proof supporting that it represents "average input energy".} } is equivalent to the ``average input energy'' of the closed-loop system with the policy $u_t = Kx_t$ --- the norm of $K$ in the normal Euclidean metric does not provide such relevance. \lina{since this section is only a high level of motivation, this technical paragraph may be deferred to later section. Consider just wrapping up the message into 2 high-level sentences. Otherwise, we either need to repeat the technical presentation later or what ever discussed here may be lost/forgot.}\shahriar{Sure, how about this revised paragraph? I've also moved the details to the appropriate section}
As for dynamic policies in the case of LQG \eqref{eq:LQG_policy-optimization}, there exists an inherent \textit{symmetry} for both $\mathcal{C}_n$ and $J_{\texttt{LQG}}(\mK)$, arising from standard similarity transformations in control. A similarity transformation reflects a coordinate change for the internal state of policy \eqref{eq:controller_discrete} which neither affect the stability properties, nor the input-output performance of the closed-loop (including $J_{\texttt{LQG}}$ cost).
However, the local geometry around each point (including the gradient direction) can be drastically different due to the effect of this coordinate change. %
  
Instead, we can define an \textit{orbit} for each $\mK \in \mathcal{C}_n$, over which the LQG performance remains constant, and equip the orbit space %
with a Riemannian metric $\tensor{\cdot}{\cdot}{\mK}^{\text{KM}}$ in \eqref{eq:KM-metric} that allows relating system theoretic notions of controllability and observability Gramians to dynamic policy parameters $\mK$.\footnote{To be accurate, we will restrict ourselves to \textit{minimal} dynamic policies , denoted as $\mathcal{C}_n^{\min}$, for technical reasons.}
As a result, instead of optimizing over $\mathcal{C}_n$ that may result in some ill-conditioning due to these similarity transformation, we will discuss more efficient and numerically stable Riemannian gradient descent schemes on this Riemannian manifold in \Cref{subsection:symmetry-manifold-structures-LQG}.





